A data-flow oriented software architecture for heterogeneous marine data streams

Marine in-situ data is collected by sensors mounted on fixed or mobile systems deployed into the ocean. This type of data is crucial both for the ocean industries and public authorities, e.g., for monitoring and forecasting the state of marine ecosystems and/or climate changes. Various public organizations have collected, managed, and openly shared in-situ marine data in the past decade. Recently, initiatives like the Ocean Decade Corporate Data Group have incentivized the sharing of marine data of public interest from private companies aiding in ocean management. However, there is no clear understanding of the impact of data quality in the engineering of systems, as well as on how to manage and exploit the collected data. In this paper, we propose main architectural decisions and a data flow-oriented component and connector view for marine in-situ data streams. Our results are based on a longitudinal empirical software engineering process, and driven by knowledge extracted from the experts in the marine domain from public and private organizations, and challenges identified in the literature. The proposed software architecture is instantiated and exemplified in a prototype implementation.

==> sections/arch_in_context.tex <==
\section{Architecture in Context} %Prototype implementation architecture
\label{sec:prototype_arch}

% \begin{figure}[htb!]
%     \centering
%     % [trim={left bottom right top},clip]
%     \includegraphics[trim={5.2cm 0.3cm 0cm 0cm},clip,width=\linewidth]{figures/arch_in_context.pdf}
%     \caption{Architecture of the prototype implementation (legend in Figure~\ref{fig:legend}).\pat{can we increase the font size in the figure?}}
%     \label{fig:prototype}
% \end{figure}

\begin{figure}[htb!] % [H] forces the figure to be placed exactly where it appears in the text
	\centering % Horizontally center the figure
	\begin{subfigure}{\linewidth}
    	\centering % [trim={left bottom right top},clip]
    	\includegraphics[trim={5.2cm 0.3cm 0cm 0cm},clip,width=\linewidth]{figures/arch_in_context.pdf}
	\end{subfigure}
    \hfill
    \begin{subfigure}{\linewidth}
    	\centering % Horizontally center the figure
     % [trim={left bottom right top},clip]
	\includegraphics[trim={5.1cm 1.2cm 0cm 10.3cm},clip,width=\linewidth]{figures/notation.pdf}
	\end{subfigure}
    \caption{Architecture of the prototype implementation.}
    \label{fig:prototype}
\end{figure}

The prototype implementation presented in Figure~\ref{fig:prototype} reflects the ongoing migration process to the proposed architecture. To realize this migration, many factors come into play, making it a complex and slow process. More specifically, the cross-organizational dependency of the development and operation of different component blocks. %Secondly,  
%range checks - knowledge on the sensors - calibration and precision of measurements info
%tiers -  Hybrid cloud computing - explain figure legend - some are phisical machines other can be virtual machines since cloud resources computing services are used.
The tiers, graphically shown as \textsf{\small Tier}s, represent physical machines at the UWSN level while at the cloud level the components are allocated to hybrid clouds using private and public cloud providers.

%Regarding the tiers in the prototype architecture in Figure~\ref{fig:prototype}, while they represent physical machines at the UWSN level, at the cloud level the components are allocated to a hybrid cloud, using private and public cloud providers represented as a  \textsf{\small Tier}.

In the prototype there are currently two data producers organizations with different data acquisition and network communication setups, as we can see in Figure~\ref{fig:prototype}.
Organization 7 has in his portfolio a vertically integrated sensor (physical) platform that incorporates all the needed components for the data acquisition and network layers. There are currently two of these platforms deployed at sea and sending data approximately every 30 minutes to their control and storage platform.
While this setup avoids the use of wireless underwater communication, it also presents a single point of failure and needs to be combined with the deployment of other platforms to expand the area coverage.
While organization 8 has a more flexible setup, with a mesh of nodes distributed among the same area of interest and with adaptive roles locally coordinated by their gateway at the edge of the UWSN. There are currently two sensing nodes and one gateway sending data to their data platform approximately every hour.
    %By having underwater wireless communication between the different nodes (sensing nodes and the surface gateway), there is also a need to secure this interaction as a result of challenge CH9 (see Table~\ref{tab:challenges}).
Both organizations are using mobile networks to transmit data OTA (over-the-air) to their data platform, using the  \textsf{\small Network Carrier Gateway} component.

For the security inside the UWSN, because of the flexibility and distribution of components, there might be no wireless underwater data transmission and thus, the challenge \textbf{CH9} (see Table~\ref{tab:challenges}) associated with that link does not apply. This is the case for organization's 7 system's components architecture, employs all the needed components in the same physical system with serial or ethernet connections from the sensors to the surface gateway. On the other hand,  there could also be a mesh of nodes physically distributed, which the case of the configuration of the system for organization 8. The security inside their UWSN is provided by tailored framework that follows the NIST recommended levels of security in~\cite{nist_csf} with the focus on low overhead in the underwater communications.

%"The WMesh includes a security framework that implements encryption algorithms and digital signatures enabling the confidentiality, integrity, authentication and non-repudiation. The security framework has been designed to be tailored for the underwater communication allowing the security level recommended by the NIST with a really low overhead in the communication."

At the cloud level, the authors associated organization is responsible for the implementation of the components at the data management layer for the heterogeneous data streams ingested by the data producers' systems. The implemented  \textsf{\small Ingested Data Processing} component is currently transforming, quality controlling, and forwarding data sources ingested in JSON and XML formats by the different data producers. The data quality control, which will check whether a recently data point is good or bad. The check is triggered once a data point arrives to cope with real-time data usage requirement from data consumers. In case a data point is missing due to, for example, communication issues, sensor faults, the component generates a missing value and triggers an alarm. The quality of data is assessed by four data quality attributes as introduced in Section~\ref{sec:intrinsics_QA}. 
For the cross-organizational integration done at the cloud level, and as a consequence of the message-oriented middleware for data ingestion (AD3), provoked the development of a new way of delivering data for the existing data platform of organizations 7 and 8 (see Table~\ref{tab:partners}). These changes were  done to implement the expected behavior for the  \textsf{\small Data Pusher} component of the overall architecture presented in Figure~\ref{fig:arch}, and receiving the data as soon as it arrives on the different clouds. While for organization 7 all the efforts where done on their side to complete the migration process, in the organization 8 data integration using the push behavior, the  \textsf{\small Data Pusher} component was implemented on the data management side to bridge the data provided via their own MQTT broker. For the broker components implementation on the prototype we are using HiveMQ (\url{https://www.hivemq.com/}).
Lastly, regarding data ingestion, since the data was initially provided by organization 8 via a REST API using the  \textsf{\small Data Fetcher} component, this ingestion method can still be used to retrieve historical data or in case of down time (availability issues) on the sending or receiving components. 

For the  \textsf{\small Monitoring} component, we are monitoring Key Performance Indicators (KPI) for the data platform. These KPIs function as service level objectives and are translated to interact with the Prometheus  monitoring toolkit (\url{https://prometheus.io/}) where runtime metrics are stored.

Concerning the data provision to  \textsf{\small Data Consumer Application}s, the currently prototype is dealing with heterogeneous authentication methods challenge being in the process of migrating to a centralized authentication  method using Keycloak (\url{https://www.keycloak.org/}) identity and access management solution to enable the access control via the  services' identity associated credentials. 
Nevertheless, for testing proposes, a  \textsf{\small Data Streams Visualization} GUI has being integrated to visualize the data coming from the different streams. This component was implemented using Thingspeak (\url{https://thingspeak.com}).
%A public version of this integration with a virtual sensor stream is available in: \url{https://thingspeak.com/channels/2129424}.\thanh{The channel location shows Bergen. In Section~\ref{sec:method}, we say~\cite{ref14}, which is our IoT paper, is the starting point of our study. Would that be dangerous that the reviewers discover who we are as they can find out the authors of~\cite{ref14} are from Bergen? Would they blame us that we do not comply with the double-blind review policy?}
Finally, on the  \textsf{\small Data Consumer Application} side, efforts are being made to deliver data to a data visualization and analytics software operated by organization 2, and to a marine data archive managed by organization 13 (see Table~\ref{tab:partners}). %To accomplish this milestone, the data classification must also be performed in the  \textsf{\small Stream Processing} component.

%solutions when it comes to the automation of distributibution and update of credencial in a cross-organizational context


==> sections/archive/RE_DQ_dimensions.tex <==
%Data quality is evaluated through different sets of categories, and the two most common are extrinsic and intrinsic~\cite{haug2021understanding}. Extrinsic factors indicate how well the data serves a certain purpose in operations or decision-making. It is suitable to evaluate whether the data meets contextual needs of the use cases defined beforehand (i.e., traditional approach of marine data collection). For example, ``extrinsic meaningfulness'' indicates how well an invididual understands the data with respect to a certain real-world phenomenon or task~\cite{bovee2003conceptual}. Intrinsic factors, on the other hand, evaluate the quality of the data without considering or comparing with other information, e.g., real-world context. In that sense, ``intrinsic meaningfulness'' evaluates how independent the data from the real-world is. In general, evaluating using intrinsic factors  gives clearer and quantifiable evaluations than extrinsic ones. However, extrinsic factors give 

%Data quality is perceived as a set of dimensions, each describing a particular quality characteristic of data~\cite{haug2021understanding}. Depending on application areas, there are suitable sets of data quality dimensions. 

%There are different ways to evaluate the quality of data. One is to measure how well the data serves a certain purpose in operations or decision-making. This is called ``extrinsic data quality'' and has been used for evaluating whether the data meets requirements of the use cases defined beforehand (i.e., traditional approach of marine data collection). User perceptions also play an important factor in evaluating data quality. Distinguished from the ``extrinsic data quality'' evaluative approach is ``instrinsic''. In this case, the quality of the data is evaluated without being considered or compared with other information, e.g., real-world applications. Instrinsic data quality measurement gives clearer and quantifiable evaluations than extrinsic. For example, 

%Another way of measuring data quality is to evaluate 


The recent SLR on data quality in~\cite{haug2021understanding} highlights the importance to identify and define a set of data quality categories and dimensions in order to acknowledge existing classifications that can help better frame our research contributions in the field. When it comes to data quality categories, it is important to distinguish between intrinsic and extrinsic characteristics of data, which sometimes can result in more objective or quantifiable evaluations~\cite{haug2021understanding} for the first case, whilst the second can result in more system- or use case-specific evaluation. As for the dimensions, we are focusing on the ones typical in  IoT domains identified in~\cite{Liu2020}, and the ISO/IEC 25012 quality model for data products~\cite{iso25012}. In the intrinsics category quality can be measured in terms of: accuracy 
%(comparison of the measurement and the real-world correspondent aspect)
, timeliness, completeness (expected data), data volume, and  concordance (w.r.t. related data),~\thanh{utility?}. While in the extrinsics category, we are addressing: understandability, utility (relevance), and portability (reusability).
%, and we redirect readers to this study for further details and definitions of the dimensions.  
%In this work, we focus on the accuracy dimension of the intrinsics category which is defined as ``\textit{The extent to which an observation for the object truly reflects its real-world situation}'' in~\cite{Liu2020}. \keila{Merge definitions}

%Haug recently conducted a SLR on data quality~\cite{haug2021understanding} highlighted the importance of identifying and defining data quality categories and dimensions. Data quality categories relate to intrinsic and extrinsic characteristics of data. Clarifying intrinsic characteristics can result in more objective or quantifiable evaluations, whilst making clear extrinsic characteristics can lead to more system- or use case-specific evaluations. As for the dimensions, we are focusing on the ones typical in  IoT domains identified in~\cite{Liu2020}, and the ISO quality model for data~\cite{iso25012}. In the intrinsics category quality can be measured in terms of: accuracy 
%(comparison of the measurement and the real-world correspondent aspect), timeliness, completeness (expected data), data volume, and  concordance (w.r.t. related data). While in the extrinsics category, we are addressing: understandability, utility (relevance), and portability (reusability).
%, and we redirect readers to this study for further details and definitions of the dimensions.  
%In this work, we focus on the accuracy dimension of the intrinsics category which is defined as ``\textit{The extent to which an observation for the object truly reflects its real-world situation}'' in~\cite{Liu2020}. \keila{Merge definitions}

%Assumptions
Considering the guidelines in \cite{haug2021understanding} and the set of categories and dimensions considered above, our study addresses the definitions of data quality in the following manner: \keila{revisit later - or only use: Evaluation perspective in discussion}
\begin{itemize}
    \item Focus: we are addressing the problems around diversifying data quality requirements within the domain sector by considering data acquired by underwater sensors. Furthermore, these sensors can integrate a larger underwater and/or surface network into the Internet-of-Underwater-Things (IoUT) field.
    \item Evaluation perspective: in the lens of the existing data quality dimensions and categories identified above, our work focuses on gathering QC information that can be quantified or measured to allow to automate of QC methods for reliable data delivery and (re)usage. Despite these last two dimensions (reliability and re-usage) focus on the system, they are useless in case there is no way to understand if the measurements are correct or valid. Thus, this work falls into both intrinsics and extrinsics of data, encompassing information that can be used to assess the quality of the data w.r.t. different use cases.  
    \item Data structure: as a result of our perspective on the problem, we are considering data in unstructured and semi-structured which are closely related to the early stages of the data management lifecycle. This happens because we are focusing on the stages before archiving data where usually a data model is required. Nevertheless, understanding factors that influence the quality of data is useful for the definition of required metadata that must companion the data in order to assure its quality.
    \item Data level: finally, when it comes to levels of data, we are considering the data values, i.e. the measurement values, its fields, and relations w.r.t. quality control information for accuracy.
\end{itemize}

\begin{table}[h]
  \caption{Data Quality Categories and Dimensions\thanh{Extrinsic deals with contextual understanding of data, meaning that data should meets certain requirements for use cases. It is something we want to address in this paper and make the data applicable in most cases. I was wondering if we should ignore these categories. For intrinsic category, I agree that utility will be ignore as it deals with data quality between databases and data consumers. Out of scope of this paper.}}
  \label{tab:DataQuality}
  {\small
\begin{tabular}{|l|l|l|}
\hline
Dimension & Category & Definition \\ \hline
Accuracy & \multirow{5}{*}{intrinsics} &  \\ \cline{1-1} \cline{3-3} 
Timeliness &  &  \\ \cline{1-1} \cline{3-3} 
Completeness &  &  \\ \cline{1-1} \cline{3-3} 
data volume &  &  \\ \cline{1-1} \cline{3-3} 
concordance &  &  \\ \hline
understandability & \multirow{3}{*}{extrinsics} &  \\ \cline{1-1} \cline{3-3} 
utility (relevance) &  &  \\ \cline{1-1} \cline{3-3} 
portability (reusability) &  &  \\ \hline
\end{tabular}
}
\end{table}

==> sections/archive/abstract.tex <==
%IoUT are IoT systems composed by an UWSN on its data production layer. This data acquision component is exactly what makes this systems so unique, which data-related components can be managed by different organization from the ones owning and making decsions on the collected data and its sharing for reusability outside of the operational scenario which the system is deployed.
Marine in situ data, i.e., data that is collected locally inside of the water by sensors mounted on fixed or mobile systems is crucial for understanding and forecasting marine ecosystems' state and climate. In the past decade, several public organizations have collected, managed, and shared this type of data openly. Furthermore, this type of data is also valuable for companies operating at sea, including those in the oil and gas industry, aquaculture, wind production, and maritime transport. More recently, initiatives such as the Ocean Decade Corporate Data Group have incentivized the sharing of data of public interest from private companies in the same way, aiding also in the management of the oceans.
This paper presents an ongoing long-term empirical software architecture development process to integrate, process, and share data in a cross-organizational setting composed of stakeholders from public and private organizations working in the marine domain. The research process is based on the knowledge extracted from the stakeholders' experience and challenges found in the literature on building systems in this environment characterized by limited resources where data is generated. The challenges were analyzed regarding their impact on the overall system's software and data quality attributes. As a result of our process, we present architectural decisions to address the challenges. Furthermore, we propose a software architecture focused on those challenges that highlight the data flows from the different organizations. Lastly, as part of our validation process, we present a prototype implementation of the proposed architecture in this context.%, contributing solutions to collaborative ways of integrating and using data.

==> sections/archive/challenges.tex <==
\section{Challenges}\label{sec:challenges} %Challenges Gathering
This section discusses challenges of building \texttt{System} and they are divided into three layers as proposed in~\cite{ref14}: underwater data acquisition layer, network communication layer, and data management layer. \thanh{Keila, can you help to write how you survery the literature for challenges?} Table~\ref{tab:challenges} summarizes the challenges, how they affect quality of software and data, and their reference source.

\thanh{Table~\ref{tab:challenges} also indicates quality of software product impacted and quality of data product impacted. The information is not available on the discussions below. Where will we deal with them?}

%present in literature throughout the data value chain in autonomous wireless stationary marine observing systems. Among the systems challenges, we focus on describing in detail the ones that are relevant to the overall software architecture, posing architecture concerns to be dealt with when developing solutions in the domain of application. The challenges are divided into three layers of a typical Internet of Things (IoT) system which was proposed in~\cite{ref14}, namely underwater data acquisition layer, network communication layer, and data management layer. Table~\ref{tab:challenges} summarizes the challenges, how they affect quality quality of software and data, and reference source.
%~\thanh{Keila, some citations for the model that you picked here, please},

\subsection{Underwater Data Acquisition Layer}
\paragraph{Limited battery (CH1)} The only power source for underwater equipment is battery. In general, its resource is limited and varies from a few weeks to two years depending on many factors, including data sampling rate and the quality of instruments. This challenge forces software embedded on sensors to consume as little power as possible, which includes managing processing and transmission tasks.

\paragraph{Physical vulnerability (CH2)} Equipment to collect data (underwater sensors) and transmit the data to the shore (underwater communication modems or hubs) are vulnerable to physical impacts. For example, the equipment can be damaged by human activities (e.g., hit by ships) or by nature (e.g., dragged around by sea ice). In such cases, bad data is generated. In the worst scenario, the whole IoUT can be destroyed.

\paragraph{Lack of device output format standards (CH3)} There are many underwater sensor manufacturing companies and they do not have an agreement on how to represent data. They also employ different communication protocols. This problem obstructs interoperability between sensor families and data collected by different data producers. %Interoperability (plug and play)
%efficiency from \cite{bass2003software} and 2 pilars of sustainability mentioned in~\cite{VENTERS2018174}


\paragraph{IoUT equipment environmental impact (CH4)} Placing underwater equipment in the sea would affect the behaviour of marine animals. There are regulations regarding how dense the equipment is deployed to keep the ocean sustainable. The regulations may affect the quality of data received at the end.

\subsection{Network Communication Layer}
\paragraph{Unreliable UAC links (CH5)} UAC has low communication bandwidth and high propagation delay, especially with horizontal communication as the signals are prone to distortions.% The more UAC is used to communicate between underwater equipment horizontally, the more errors the technology incur. 

\paragraph{Missing raw data (CH6)} Employing UAC has both pros and cons for \texttt{System}. On the one hand, \texttt{System} is cheaper to build compared to utilizing submarine optic cables. On the other hand, UAC has low communication bandwidth and high propagation delay. Transmitting live images of the sea or multi-parameter marine data in real-time are almost impossible. To deal with this challenge, \texttt{System} has to selectively transmit important information. It leads to the challenge that data consumers cannot obtain raw data for their data analytics tasks or lack of error recovery ability.

\paragraph{Environmental impact of UAC (CH7)} The more data transmitted via UAC links, the more noise generated in the ocean. Such phenomenon will confuse marine animals and affect their behaviors.







\paragraph{Low communication bandwidth and high operation cost of satellite links (CH8)} Not only UAC has low communication bandwidth but also satellite, which is responsible for transmitting data from sea surface communication hubs to the shore, does. In addition, the more satellite links are used, the more operation cost to be used as in general it is expensive.
%\thanh{for me, CH8 and CH9 can be merged together like the IoT paper. I write the challenge in that way but feel free to change to you want to split.} 

\paragraph{Security vulnerability of UAC links (CH9)} Most of marine data is represented in the time-series format. In general, they are small in size. However, when the data is encrypted, its size will increase and imposes burden on UAC links which have low communication bandwidth.

\paragraph{Power hungry UAC data transmission (CH10)} Data transmission over UAC can drain battery of underwater equipment quickly. This constraint forces ocean observation systems to transmit as little data as possible to reserve this only power supply source.



\subsection{Data Management Layer}
\paragraph{Complex data usage (CH11)} There are many types of marine data collected (e.g., data series, images, or videos). The data can be used in many applications, which data producers tailor to specific needs. Because of that, marine data is complicated to interact with and usually require data consumers to have certain levels of domain knowledge.

\paragraph{Lack of automatic QC procedures (CH12)} Marine data is prone to errors to due various environment impacts and technological constraints. For example, biofouling is the growing of microorganisms around underwater sensors. It is an unavoidable problem for artificial objects operating in the ocean. When a sensor experience that issue, it will produce inaccurate data. Besides, existing communication technologies are unreliable and may generate noise during data transmission. It is important to perform data quality control before employing the data further. However, due to high complexity of data and diverse ways to represent the data, such activities are done by only domain experts and usually delay by up to six months. In addition, the practitioners admitted that performing data quality control is subjective and mostly based on perspectives and experience of the person in charge. 

\paragraph{Absence of common data platforms (CH13)} Marine data producers store data at different places depending on their needs and capacity. 
%Introducing a common data platform is not an easy work as there are conflicts of interest. 
Specifically, data collected by public research institutes are usually open, but it is not the case for companies. For the latter, the data is stored in private servers and not open to the public. 
%Mention that most of the literature focus on delivering the data to the cloud side reliably but not so much on how the data processment, storage and sharing (data management) is performed for the use cases in the application domain.

%\subsection{Application layer}
\paragraph{Filter sensitive data (CH14)} There are many activities happening simultaneously in the ocean. Due to regulations, a large amount of marine must not be shared to the public, such as submarine activities and stock-sensitive information. Public data producers have to selectively filter the data based on regulations and their data usage patterns.

%\paragraph{Lack of marketplace for data sharing and selling (CH15)}
\paragraph{Lack of mechanisms for data sharing and selling (CH15)}
There are conflicts of data producers regarding business models for managing the data. While public data producers prefer the data to be accessible to the public, companies want to monetize the data as it is costly to collect. It is important to have a marketplace where data consumers can access the data they want and pay for it if required. 
%enforcement of the sharing rules and policies to operations and decision-making systems, regulatory data delivery, or data reusability in open-data platforms.

\paragraph{Access control for data sharing (CH16)} There are certain marine data categories that are restricted to public data consumers even with commercial deals. Access control must be enforced to ensure only the right consumers can access to data shared by \texttt{System}.



%\keila{Low resources, raw data, low bandwidth, costly comms, security, data platform, data sharing}
%\keila{(Papers on IoTJ + 3 papers) + Our workshops on our method}

\begin{table*}[h]
\caption{Software architecture relevant challenges on stationary wireless marine observing systems}
\label{tab:challenges}
\centering
\scriptsize
{
\centering
\begin{tabular}{|c|l|c|l|ll|l|}
\hline
\multirow{2}{*}{\textbf{ID}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Challenge}}} & \multirow{2}{*}{\textbf{Layer}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Quality of Software \\ Product Impacted\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Quality of Data Product Impacted}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{References}}} \\ \cline{5-6}
 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{Inherent}} & \multicolumn{1}{c|}{\textbf{System-dependent}} & \multicolumn{1}{c|}{} \\ \hline
CH1 & Limited battery & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Underwater \\ Data Acquisition\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Energy efficiency* \\ Reliability (availability)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility, \\ Accuracy\end{tabular}} & Availability & \cite{ref2,ref3,ref5,ref11,ref13,ref14} \\ \cline{1-2} \cline{4-7} 
CH2 & Physical vulnerability &  & Reliability (availability) & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility, \\ Consistency\end{tabular}} & Availability & \cite{ref3,ref4,ref5,ref7,ref8,ref11,ref14} \\ \cline{1-2} \cline{4-7} 
CH3 & Lack of device output format standards &  & Compatibility (Interoperability) & \multicolumn{1}{l|}{Credibility} & Compliance & \cite{ref3,ref5,ref7,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
\multicolumn{1}{|l|}{CH4} & IoUT equipment environmental impact &  & Energy efficiency* & \multicolumn{1}{l|}{Credibility} & Compliance &  \\ \hline
CH5 & Unreliable UAC links &  & Reliability & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness\end{tabular}} & Availability & \begin{tabular}[c]{@{}l@{}} \cite{ref2,ref4,ref5,ref7,ref9} \\ \cite{ref10,ref11,ref14} \end{tabular} \\ \cline{1-2} \cline{4-7} 
CH6 & Missing raw data &  & Explainability* & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness\end{tabular}} & \begin{tabular}[c]{@{}l@{}} Availability \\ Understandability\end{tabular}  & \cite{ref13,ref14} \\ \cline{1-2} \cline{4-7} 
CH7 & Environmental impact of UAC & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Network \\ Communication\end{tabular}} & Energy efficiency* & \multicolumn{1}{l|}{Credibility} & Compliance & \cite{ref1,ref5,ref14} \\ \cline{1-2} \cline{4-7} 
CH8 & \begin{tabular}[c]{@{}l@{}}Low communication bandwidth and \\ high operation costs of satellite link\end{tabular} &  & \begin{tabular}[c]{@{}l@{}}Performance efficiency \\ (capacity and resource utilization)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility, \\ Currentness, \\ Completeness\end{tabular}} & Availability & \cite{ref6,ref13,ref14,ref16} \\ \cline{1-2} \cline{4-7} 
CH9 & Security vulnerability of UAC links &  & Security & \multicolumn{1}{l|}{Credibility} & Confidentiality & \cite{ref3,ref6,ref11,ref12,ref14} \\ \cline{1-2} \cline{4-7} 
CH10 & Power-hungry UAC data transmission &  & Energy efficiency* & \multicolumn{1}{l|}{Credibility} & Availability & \cite{ref3,ref10,ref14} \\ \hline
CH11 & Complex data usage & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Data \\ Management\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Compatibility (Interoperability), \\ Usability \\ (Appropriateness recognizability)\end{tabular} & \multicolumn{1}{l|}{N/A} & Understandability & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
CH12 & Lack of automatic QC procedures &  & Explainability* & \multicolumn{1}{c|}{\textbf{All}} & \multicolumn{1}{c|}{\textbf{All}} & \cite{ref13,ref14,ref15,ref17} \\ \cline{1-2} \cline{4-7} 
CH13 & Heterogeneous data sources & & \begin{tabular}[c]{@{}l@{}}Compatibility (Interoperability) \\ Usability (Operability)\end{tabular} & \multicolumn{1}{l|}{N/A} & Accessibility & \cite{ref13,ref15,ref18} \\ \cline{1-2} \cline{4-7} 
CH14 & \begin{tabular}[c]{@{}l@{}}Sensitive data \\ (Business and Defense critical)\end{tabular} &  & Security & \multicolumn{1}{l|}{N/A} & \begin{tabular}[c]{@{}l@{}}Confidentiality, \\ Compliance\end{tabular} & \cite{ref13,ref15} \\ \cline{1-2} \cline{4-7} 
%CH15 & \begin{tabular}[c]{@{}l@{}}Lack of marketplace for \\ data sharing and selling\end{tabular} &  & Usability (accessibility - of data) & \multicolumn{1}{l|}{N/A} & Accessibility & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7}
CH15 & \begin{tabular}[c]{@{}l@{}}Lack of mechanisms for data sharing\\ and selling (data reusability)\end{tabular} &  & Usability & \multicolumn{1}{l|}{N/A} & Accessibility & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
CH16 & Access control for data sharing &  & Security & \multicolumn{1}{l|}{N/A} & Confidentiality & \cite{ref13,ref15} \\ \hline
\end{tabular}
}
\begin{tablenotes}
      \item \small
     \hspace{.1cm}
*  -- New QA

\end{tablenotes}
\end{table*}
%\keila{complement CH3 and CH11 with RE paper Fig2: Lack of interoperability among different sensors and system output data}
%\keila{Number challenges w.r.t. surveyed papers and have one column to refer if it was mention in our meetings}

%Data (re)usability: sharing or selling marketplace

==> sections/archive/challenges_full.tex <==
\section{Challenges}
\label{sec:challenges}
In this section, we introduce software and data product quality attributes from standardized quality models. Since these standardized models are not able to capture all the impacting concerns from the identified challenges, additional quality attributes from the literature are adopted for the purpose. Those are described in section~\ref{sec:QA}.
Lastly, we describe main quality attributes negatively impacted by the identified challenges, describing their effect on the resulting software architecture. Table~\ref{tab:challenges} summarizes a total of fifteen challenges that were identified and analysed in terms of its impact to software and data quality attributes following the ISO/IEC standards. For the latter, the attributes are spread across three categories: inherent data quality (accuracy, completeness, consistency, currentness, and credibility), inherent and system-dependent data quality (accessibility, efficiency, compliance, confidentiality, precision, traceability, and understandability), and system-dependent data quality (availability, portability, and recoverability).
We have aggregated and discussed the impact on software quality attributes in conjunction with the last two data quality categories because of the perceived intersectionality among them. We complete the section with the discussion of impacted data inherent quality attributes in section~\ref{sec:intrinsics_QA}.
%%Because of the intersectionality among the last two data quality dimensions quality attributes and the software ones, we have aggregated and discussed them by the software quality attributes. %discuss from image in: https://link.springer.com/article/10.1007/s11219-019-09494-x/figures/2
\subsection{\del{Quality Attributes}}
\label{sec:QA}
Because of the system's behavior dependence on data quality when analysing an architecture in the point of view of its heterogeneous data flows, we have analyzed the gathered challenges with regards to quality attributes for software and data products from the ISO/IEC 25010~\cite{iso25010} and the ISO/IEC 25012~\cite{iso25012} quality models respectively. There was a need to introduce two more quality attributes on the software quality model for accommodating challenges' concerns not captured by the existing ones. More specifically, we borrow the Energy efficiency suggested in~\cite{bass2003software} and Explainability from~\cite{9609199,habibullah2023non}. 
While the sustainability of architectural decisions remain an open challenge and relates to the evolution of systems~\cite{VENTERS2018174}, characteristics such systems' energy efficiency~\cite{bass2003software,VENTERS2018174,koccak2015integrating} are identified across different studies as quality attributes to consider when evaluating software systems. Even though the ISO/IEC 25010~\cite{iso25010} encompasses a resource utilization sub-characteristic under performance efficiency quality attribute, these usually refer to computational resources (e.g. CPU, storage, and network usage) which can be ambiguous if energy is perceived as a ``resource'' because it is a trade-off to the computational resources. 
%\keila{This new restructuring only has 2 less sub-subsections that the previous challenges list description version in sections/challenges.tex}
Explainability has emerged as quality attribute associated to machine learning and other AI-based components because of their associated ``black box'' characteristics. This attribute appears often associated with the quality of data used by such systems because of its runtime behavior dependency on data~\cite{9609199} and the influence it has on the decision-making process of these systems. In this work we adopt this quality attribute having this definition in mind.

% \subsection{Software Product and Data Product System-dependent Quality Attributes Impacted}
% \label{sec:system_QA}
%\keila{Merging both attributes because of their intersectionality}

%\paragraph{Compatibility}
\subsection{Compatibility}
\label{sec:compatibility}
Concerning \textbf{compatibility} between interacting components in the system, some concerns affect the interoperability in two different layers. Firstly, at the underwater data acquisition layer, because of the sensor integration, heterogeneous communication protocols and associated output data formats need to be unified at the UWSN level to ensure a common understanding within data producers' sub-systems (challenge \textbf{CH3}: lack of device output format standards). Secondly, at the data management layer, the originated dataset from the integration of measurements from different sensors is supplied by data producers' sub-systems in various formats (syntax) with fields differing in their meaning semantics. Additionally, there might be different types of data, such as time series, images, or videos, which are categorized into point-based and array-based data~\cite{ref15}. At the cloud level, where multiple data sources are merged, it is necessary to make them interoperable to ensure that the different processing components interpret data based on the same metrics and criteria (challenge \textbf{CH12}: Heterogeneous data sources).
When data has proprietary or organization-dependent syntax and semantics, its \textbf{compliance} to standards  and \textbf{portability} (i.e., ``\textit{degree to which data has attributes that enable it to be installed, replaced or moved from one system to another}'') can be affected.

%\paragraph{Explainability and Usability}
\subsection{Explainability and Usability}
\label{sec:explainability}
Because of the low communication bandwidth and high propagation delay of UAC at the UWSN level, there is often processing and aggregation of data sending only what is consider important information or events up the data delivery chain. The raw data is often kept for retransmission and can be retrieved at recovery or maintenance of the sensing platforms at sea. Despite that, storage might also be an issue when operating for long time. Since the raw records can be crucial for data analytics tasks, their absence can have implications in the \textbf{understandability} of data and the \textbf{explainability} of automatically detected phenomena or actions  performed based on the data (challenge \textbf{CH5}: missing raw data). Another challenge affecting the \textbf{understandability} of data is complex data usage derived from the lack metadata that can provide information regarding the required data quality intrinsic (inherent) dimensions hindering its adequate use for a specific context (challenge \textbf{CH10}). In the end user application side, this challenges impacts the \textbf{usability} (Appropriateness recognizability), and more specifically the ability to ``\textit{recognize whether a product or system is appropriate for their needs}''. On the other hand, the lack of data quality control (challenge \textbf{CH11}) procedures also impacts the \textbf{explainability} because of the high complexity of data and diverse ways to represent the data, such activities are done by only domain experts and usually delay by up to six months. In addition, the practitioners admitted that performing data quality control is subjective and mostly based on perspectives and experience of the person in charge. Most of the existing procedures focus on assessing the intrinsic characteristics of data because marine data is prone to errors to due various environment impacts and technological constraints. Besides, existing communication technologies are unreliable and may generate noise during data transmission. Therefore, it is important to perform data quality control before employing the data further considering \textbf{all the quality dimensions required for its context of use}.

%\paragraph{Reliability and Performance efficiency}
\subsection{Reliability and Performance efficiency}
\label{sec:reliability}
Regarding \textbf{performance efficiency}, because of the impact of the underwater acoustic signals used by the communication devices into the marine life, there might be restrictions to the transmission windows and frequencies according to the ecosystem surrounding the operations infrastructure at sea. This challenge has implications to the communication channels and links utilization (\textbf{resource utilization}). Furthermore, the noise generated by the communication device's signals can negatively impact species that use acoustics to communicate or prey leading to confusion or other changes in behavior of the animals (challenge \textbf{CH6}). %As a consequence, this constraint can impact the \textbf{availability} of data.

When it comes to \textbf{reliability} at the underwater data acquisition layer, the only power source for underwater equipment is the battery. This limited resource lifetime can vary from a few weeks to two years depending on many factors, including data sampling rate and the precision of instruments. This challenge forces software embedded in sensor nodes to optimize power consumption, which includes managing processing and transmission tasks. Regarding these tasks, there are indications that transmission devices consume more energy than computation, and components can be temporarily powered off to save energy (sleep mode)~\cite{ref14}.
Furthermore, at this layer, equipment to collect data (underwater sensors) and transmit the data to the shore (underwater communication modems or gateways) are vulnerable to physical impacts. For example, the equipment can be damaged by human activities (e.g., hit by ships) or by nature (e.g., dragged by sea waves, currents, or ice). In such cases, sensors' measurements or even integrity and their resulting data can be affected. 
On the other hand, in the network communication layer, underwater acoustic communication (UAC) has low communication bandwidth, high propagation delay, and high bit error especially with horizontal communication, as the signals are prone to distortions. The water conditions may also deteriorate the signal propagation, which is already very constrained. Furthermore, wireless communication channels in IoUT have less available bandwidth per packet transmission (challenge \textbf{CH7}) than land-based or IP networks. This is the case for the acoustics for underwater communications and satellite for over-the-air communication (OTA) which latency can vary according to atmospheric or water conditions (e.g. affected by absorption). These challenges constraints the overall network \textbf{performance efficiency capacity} quality attribute in the software systems in IoUT environment. Lastly, regarding the communication channels, the OTA options (satellite and mobile networks) to transmit data into IP network usually has higher costs associated to the carrier service.
In summary, while the physical vulnerability (challenge \textbf{CH2}) of the hardware and the limited battery (challenge \textbf{CH1}) affects the availability of the software system (its operation), the unreliability associated with the wireless underwater network links (challenge \textbf{CH4}: Unreliable UAC links) impacts the capacity of the software system to operate despite the faults in the communication channel. %recoverability implication as well 
Overall, these challenges impact the \textbf{recoverability}, i.e., its ``\textit{degree to which data has attributes that enable it to maintain and preserve a specified level of operations and quality, even in the event of failure}''.
Moreover, another challenge whose failure could impact data availability are the power-demanding UAC transmissions (challenge \textbf{CH9}). %\paragraph{Energy efficiency}
Transmissions must be handled carefully to avoid the quick drainage of the battery power because communication devices can be the component that consumes more energy in the systems at the UWSN level. As pointed out in~\cite{bass2003software}, \textbf{energy efficiency} of software systems can no longer be disregarded. In the marine domain, it is one of the main drivers of the overall system because of its implication on the availability of the systems and the data produced by them due to the risk of power down and the time and costs to its maintenance (e.g. battery replacement operations). 

%\paragraph{Security}
\subsection{Security}
\label{sec:security}
Regarding \textbf{security} at the network communication layer, the open wireless communication channel usually done via UAC is susceptible to a range of interference (challenge \textbf{CH8}) which can lead to the capturing of transmitted packages (routing attacks) or blockage of a link between nodes (DoS). As any other network, authentication should be done but the land based network authentication methods implementation in this context is not trivial due to the communication overhead. Other detection and mitigation can be implemented to circuvein the openness of the communication channel but those increases the communication overhead underwater which is already restricted, specially in the case where there are many nodes in the network. For more detailed description of the types of attack and their mitigation, we redirect readers to~\cite{ref19}.  At the data management layer there are two interrelated challenges impacting the security in terms of the confidentiality and the rightful access to data being shared. The access to data being being collected needs to be carefully filtered in terms of its category (challenge \textbf{CH15}). Because of the need to share data beyond the initial context it was acquired motivated by regulations, better forecast and safety measures on organizations' operations areas, or to adhere to initiatives to provide data for climate and marine sciences for better public perception (challenge \textbf{CH14}: data reusability). In summary the data to be shared could be categorized into (challenge \textbf{CH13}):
    \begin{itemize}
        \item \textbf{Legally restricted} -- Data that cannot or has to be shared to compliance with laws and regulations. An example is data that is critical for the maritime territory defence of a country because it details the bathymetry of a specific region at sea.
        \item \textbf{Business critical} -- Data that contains critical information for business operations, e.g. ``sensitive data''. This type of data is critical not only for data owners but also for data producers to improve sensor measurements at the data acquision layer.
        \item \textbf{Resource-depending} -- Data that can cause no harm to sharing entity, e.g. ''non-footprint'',  and can be valuable to a third party entity or to new applications, but requires resources to be shared. This data, of is not being sent can be easily overwritten since storage can also be a constraint in the sensing devices or at the gateways in the edge.
    \end{itemize}
In terms of data-related quality attributes, these challenges impacts \textbf{availability}, i.e. ``\textit{the degree to which data has attributes that ensure that it is only accessible and interpretable by authorized users}''; and \textbf{confidentiality} which is defined as ``\textit{The degree to which data has attributes that enable it to be retrieved by authorized users and/or applications}''.

\subsection{Data Product Inherent Quality Attributes Impacted}
\label{sec:intrinsics_QA}
% \keila{use RE table}
\paragraph{Accuracy}
This quality attribute is impacted by all challenges that affect the sensor measurements, deviating the measurements from the observed phenomena tried to be captured. For example, biofouling is the growing of microorganisms around underwater sensors. It is an unavoidable problem for artificial objects operating in the ocean. When a sensor experience that issue, it will produce \textbf{inaccurate} measurements that can lead to errors such as data drift. Another example of factors impacting data accuracy is the sensor power supply, if battery is running low and there are inconsistencies to the sensor energy supply, there might be errors introduced in the sensors' readings which originates ``bad'' data. Lastly, the physical vulnerability also affects the positioning of the sensors and thus can have an negative implication on the reading. An example of such are for sensors deployed close to the water surface, in case they make a reading outside of the water. Another case could be the sensors using their static configured position as part of the data acquisition and are dragged from their initially deployed location.

\paragraph{Completeness, Consistency and Currentness}
These quality attributes are impacted by all challenges affecting the reliability and performance (in terms of network throughput) quality attributes of the data-producing system at the data acquisition and network communication layers since the challenges entangle the availability of software components and data transmission. The compatibility-related challenges can affect the \textbf{completeness} of the data products because the lack of common fields and metadata available from the heterogeneous sources of data at the data acquisition and management layers. In addition to the compatibility challenges,  \textbf{consistency} with other data might be affected as well because of the correlation of measurements.
%Additionally, when the \textbf{completeness} is affected in this context, because of the correlation of measurements the \textbf{consistency} with other data might be affected as well. 
Finally, the high latency associated with the underwater and OTA communication channels greatly impacts the time of arrival of data to data consumer applications affecting the \textbf{currentness} data quality attribute.

\paragraph{Credibility}
We consider credibility a cross-cutting inherent data quality attribute because of the definition gave in the standard and its relation to ``\textit{truthfulness of origins}''. In the IoUT context it is not possible to have ground truth to all measurements and the most of the quality control procedures focus on investigating the closeness of the data to its true value~\cite{ref17} covering the inherent characteristics of data. Regarding the trust, other studies have also considered it as impacting at the cross-organizational level of the system because of all the uncertainty affecting the data streams until its (re)usage~\cite{ref13}.
%In contrast other studies consider credibility as an attribute related to systems' trust and thus recommend that it must be perceived as an external quality attribute (system-dependent).
This topic needs to be further investigated as it remains an open-challenge in the software and data quality research, and goes beyond the scope of this paper.

\begin{table*}[h]
\caption{Software architecture relevant challenges on stationary wireless marine observing systems}
\label{tab:challenges}
\centering
\scriptsize
{
\centering
\begin{tabular}{|c|l|c|l|ll|l|}
\hline
\multirow{2}{*}{\textbf{ID}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Challenge}}} & \multirow{2}{*}{\textbf{Layer}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Quality of Software \\ Product Impacted\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Quality of Data Product Impacted}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{References}}} \\ \cline{5-6}
 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{Inherent}} & \multicolumn{1}{c|}{\textbf{System-dependent/Both}} & \multicolumn{1}{c|}{} \\ \hline
CH1 & Limited battery & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Underwater \\ Data Acquisition\end{tabular}} & Reliability (availability)& \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Accuracy,\\ Credibility,\\Completeness\end{tabular}} & Recoverability & \cite{ref2,ref3,ref5,ref11,ref13,ref14} \\ \cline{1-2} \cline{4-7} 
CH2 & Physical vulnerability &  & Reliability (availability) & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Accuracy,\\ Credibility,\\Completeness\end{tabular}} & Recoverability & \cite{ref3,ref4,ref5,ref7,ref8,ref11,ref14} \\ \cline{1-2} \cline{4-7} 
CH3 & Lack of device output format standards &  & \begin{tabular}[c]{@{}l@{}} Compatibility \\ (Interoperability)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness,\\Consistency\end{tabular}}  & \begin{tabular}[c]{@{}l@{}} Compliance \\ Portability\end{tabular} & \begin{tabular}[c]{@{}l@{}} \cite{ref3,ref5,ref7} \\ \cite{ref14,ref15} \end{tabular} \\ \hline % \cline{1-2} \cline{4-7} 
%\multicolumn{1}{|l|}{CH3} & IoUT equipment environmental impact &  & \begin{tabular}[c]{@{}l@{}}Performance efficiency \\ (resource utilization)\end{tabular} & \multicolumn{1}{l|}{Credibility} & Compliance &  \\ \hline
CH4 & Unreliable UAC links &  & \begin{tabular}[c]{@{}l@{}} Reliability (Fault \\Tolerance) \end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\Completeness\end{tabular}} & Recoverability & \begin{tabular}[c]{@{}l@{}} \cite{ref2,ref4,ref5,ref7} \\ \cite{ref9,ref10,ref11,ref14} \end{tabular} \\ \cline{1-2} \cline{4-7} 
CH5 & Missing raw data & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Network \\ Communication\end{tabular}}  & Explainability* & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness\end{tabular}} & Understandability  & \cite{ref13,ref14} \\ \cline{1-2} \cline{4-7} 
CH6 & Environmental impact of UAC & & \begin{tabular}[c]{@{}l@{}}Performance efficiency \\ (resource utilization)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\Completeness\end{tabular}} & N/A & \cite{ref1,ref5,ref14} \\ \cline{1-2} \cline{4-7} 
CH7 & \begin{tabular}[c]{@{}l@{}}Low communication bandwidth and \\ high latency of UAC and OTA links\end{tabular} &  & \begin{tabular}[c]{@{}l@{}}Performance efficiency \\ (capacity)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility, \\ Currentness\end{tabular}} & N/A & \cite{ref6,ref13,ref14,ref16} \\ \cline{1-2} \cline{4-7} 
CH8 & Security vulnerability of UAC links &  & Security & \multicolumn{1}{l|}{Credibility} & \begin{tabular}[c]{@{}l@{}}Availability, \\ Confidentiality\end{tabular} & \begin{tabular}[c]{@{}l@{}} \cite{ref3,ref6,ref11,ref12} \\ \cite{ref14,ref19} \end{tabular} \\ \cline{1-2} \cline{4-7} 
CH9 & Power-hungry UAC data transmission &  & Energy efficiency* & \multicolumn{1}{l|}{Credibility} & Recoverability & \cite{ref3,ref10,ref14} \\ \hline
CH10 & Complex data usage & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Data \\ Management\end{tabular}} & \begin{tabular}[c]{@{}l@{}} Usability (Appropriateness \\ recognizability)\end{tabular} & \multicolumn{1}{l|}{N/A} & Understandability & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
CH11 & Lack of automatic QC procedures &  & Explainability* & \multicolumn{1}{c|}{\textbf{All}} & \multicolumn{1}{c|}{\textbf{All}} & \cite{ref13,ref14,ref15,ref17} \\ \cline{1-2} \cline{4-7} 
CH12 & Heterogeneous data sources & &  \begin{tabular}[c]{@{}l@{}} Compatibility \\ (Interoperability)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness,\\Consistency\end{tabular}} & \begin{tabular}[c]{@{}l@{}} Compliance \\ Portability\end{tabular} & \cite{ref13,ref15,ref18} \\ \cline{1-2} \cline{4-7} 
CH13 & \begin{tabular}[c]{@{}l@{}}Sensitive data \\ (Business and Defense critical)\end{tabular} &  & Security & \multicolumn{1}{l|}{N/A} & \begin{tabular}[c]{@{}l@{}}Availability, \\ Confidentiality\end{tabular} & \cite{ref13,ref15} \\ \cline{1-2} \cline{4-7} 
%CH15 & \begin{tabular}[c]{@{}l@{}}Lack of marketplace for \\ data sharing and selling\end{tabular} &  & Usability (accessibility - of data) & \multicolumn{1}{l|}{N/A} & Accessibility & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7}
CH14 & Data reusability &  & Reusability & \multicolumn{1}{l|}{N/A} & \begin{tabular}[c]{@{}l@{}}Availability, \\ Confidentiality\end{tabular} & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
CH15 & Access control for data sharing &  & Security & \multicolumn{1}{l|}{N/A} & \begin{tabular}[c]{@{}l@{}}Availability, \\ Confidentiality\end{tabular} & \cite{ref13,ref15} \\ \hline
\end{tabular}
}
\begin{tablenotes}
      \item \small
     \hspace{.1cm}
*  -- New QA

\end{tablenotes}
\end{table*}

==> sections/archive/challenges_table.tex <==
\begin{table*}[h]
\caption{Software architecture relevant challenges on stationary wireless marine observing systems}
\label{tab:challenges}
\centering
\scriptsize
{
\centering
\begin{tabular}{|c|l|c|l|ll|l|}
\hline
\multirow{2}{*}{\textbf{ID}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Challenge}}} & \multirow{2}{*}{\textbf{Layer}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Quality of Software \\ Product Impacted\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Quality of Data Product Impacted}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{References}}} \\ \cline{5-6}
 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{Inherent}} & \multicolumn{1}{c|}{\textbf{System-dependent}} & \multicolumn{1}{c|}{} \\ \hline
CH1 & Limited battery & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Underwater \\ Data Acquisition\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Energy efficiency* \\ Reliability (availability)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility, \\ Accuracy\end{tabular}} & Availability & \cite{ref2,ref3,ref5,ref11,ref13,ref14} \\ \cline{1-2} \cline{4-7} 
CH2 & Physical vulnerability &  & Reliability (availability) & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility, \\ Consistency\end{tabular}} & Availability & \cite{ref3,ref4,ref5,ref7,ref8,ref11,ref14} \\ \cline{1-2} \cline{4-7} 
CH3 & Lack of device output format standards &  & Compatibility (Interoperability) & \multicolumn{1}{l|}{Credibility} & Compliance & \cite{ref3,ref5,ref7,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
\multicolumn{1}{|l|}{CH4} & IoUT equipment environmental impact &  & Energy efficiency* & \multicolumn{1}{l|}{Credibility} & Compliance &  \\ \hline
CH5 & Environmental impact of UAC & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Network \\ Communication\end{tabular}} & Energy efficiency* & \multicolumn{1}{l|}{Credibility} & Compliance & \cite{ref1,ref5,ref14} \\ \cline{1-2} \cline{4-7} 
CH6 & Missing raw data &  & Data Quality?* & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness\end{tabular}} & Availability & \cite{ref13,ref14} \\ \cline{1-2} \cline{4-7} 
CH7 & Unreliable UAC links &  & Reliability & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness\end{tabular}} & Availability & \begin{tabular}[c]{@{}l@{}} \cite{ref2,ref4,ref5,ref7,ref9} \\ \cite{ref10,ref11,ref14} \end{tabular} \\ \cline{1-2} \cline{4-7} 
CH8 & \begin{tabular}[c]{@{}l@{}}Low communication bandwidth and \\ high operation costs of satellite link\end{tabular} &  & \begin{tabular}[c]{@{}l@{}}Performance efficiency \\ (capacity and resource utilization)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility, \\ Currentness, \\ Completeness\end{tabular}} & Availability & \cite{ref6,ref13,ref14,ref16} \\ \cline{1-2} \cline{4-7} 
CH9 & Security vulnerability of UAC links &  & Security & \multicolumn{1}{l|}{Credibility} & Confidentiality & \cite{ref3,ref6,ref11,ref12,ref14} \\ \cline{1-2} \cline{4-7} 
CH10 & Power-hungry UAC data transmission &  & Energy efficiency* & \multicolumn{1}{l|}{Credibility} & Availability & \cite{ref3,ref10,ref14} \\ \hline
CH11 & Complex data usage & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Data \\ Management\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Compatibility (Interoperability), \\ Usability \\ (Appropriateness recognizability)\end{tabular} & \multicolumn{1}{l|}{N/A} & Understandability & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
CH12 & Lack of automatic QC procedures &  & Data Quality?* & \multicolumn{1}{c|}{\textbf{All}} & \multicolumn{1}{c|}{\textbf{All}} & \cite{ref13,ref14,ref15,ref17} \\ \cline{1-2} \cline{4-7} 
CH13 & Heterogeneous data sources & & \begin{tabular}[c]{@{}l@{}}Compatibility (Interoperability) \\ Usability (Operability)\end{tabular} & \multicolumn{1}{l|}{N/A} & Accessibility & \cite{ref13,ref15,ref18} \\ \cline{1-2} \cline{4-7} 
CH14 & \begin{tabular}[c]{@{}l@{}}Sensitive data \\ (Business and Defense critical)\end{tabular} &  & Security & \multicolumn{1}{l|}{N/A} & \begin{tabular}[c]{@{}l@{}}Confidentiality, \\ Compliance\end{tabular} & \cite{ref13,ref15} \\ \cline{1-2} \cline{4-7} 
%CH15 & \begin{tabular}[c]{@{}l@{}}Lack of marketplace for \\ data sharing and selling\end{tabular} &  & Usability (accessibility - of data) & \multicolumn{1}{l|}{N/A} & Accessibility & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7}
CH15 & \begin{tabular}[c]{@{}l@{}}Lack of mechanisms for data sharing\\ and selling (data reusability)\end{tabular} &  & Usability & \multicolumn{1}{l|}{N/A} & Accessibility & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
CH16 & Access control for data sharing &  & Security & \multicolumn{1}{l|}{N/A} & Confidentiality & \cite{ref13,ref15} \\ \hline
\end{tabular}
}
\begin{tablenotes}
      \item \small
     \hspace{.1cm}
*  -- New QA

\end{tablenotes}
\end{table*}

==> sections/archive/decisions.tex <==
\begin{table}[hbt!]
\caption{Summary of Architectural Decisions}
\label{tab:decisiosn}
\centering
\scriptsize
{
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Architectural Decision}} & \multicolumn{1}{c|}{\textbf{Challenges}} & \multicolumn{1}{c|}{\textbf{QAs Impacted}} \\ \hline
AD1 & \begin{tabular}[c]{@{}l@{}}Distributed data processing\\ and transmission responsabilities\end{tabular} & \begin{tabular}[c]{@{}l@{}}CH1, CH4,\\ CH5, CH6, \\ CH8, CH10\end{tabular} &  \\ \hline
AD2 & Data platform & CH14 &  \\ \hline
AD3 & \begin{tabular}[c]{@{}l@{}}Message oriented data \\ ingestion middleware\end{tabular} & \begin{tabular}[c]{@{}l@{}}CH1, CH2, \\ CH10\end{tabular} &  \\ \hline
AD4 & MQTT messaging protocol & \begin{tabular}[c]{@{}l@{}}CH7, CH8,\\ CH10\end{tabular} &  \\ \hline
AD5 & Platform monitoring & \begin{tabular}[c]{@{}l@{}}CH1, CH2,\\ CH7, CH13, \\ CH14, CH16\end{tabular} &  \\ \hline
AD6 & Data quality control & \begin{tabular}[c]{@{}l@{}}CH6, CH12, \\ CH13\end{tabular} &  \\ \hline
AD7 & Data model for integrated data sources & \begin{tabular}[c]{@{}l@{}}CH3, CH11\\ CH13\end{tabular} &  \\ \hline
AD8 & Identity provider & CH14, CH16 &  \\ \hline
AD9 & Data sharing access control& \begin{tabular}[c]{@{}l@{}}CH14, CH15\\ CH16\end{tabular} & \\ \hline
AD10 & Data classification and triage & CH14, CH15 &  \\ \hline
\end{tabular}
}
\end{table}


==> sections/archive/intro.tex <==
\section{Introduction}
\label{sec:intro}
Marine in situ data, i.e., data that is collected locally inside the ocean by sensors mounted on fixed or mobile systems is crucial for understanding and forecasting marine ecosystems' state and climate. This type of data is also crucial for the operations in different marine industries' infrastructures installed at sea. These systems are in the origin of (near) real-time marine data streams, and they can operate for weeks and up to years without intervention because they have high associated deployment and maintenance costs. Regarding the data flow of such systems, they can be decomposed into three layers in the scope of Internet-of-Underwater-Things (IoUT)~\cite{ref14}. Firstly, there is the data acquisition layer responsible for the sensing and actuation ``things'' in or above water. Secondly, there is the network communication responsible for routing the data from \textit{ad hoc} sensor networks at sea to the IP networks, connecting the Underwater Wireless Sensor Networks (UWSN) to the internet. This layer is usually composed by a surface node that lays in the edge of the UWSN. And thirdly, there is the data management layer responsible to intermediate data delivery to applications to the different marine use cases.
If we perceive this same system in a data-related role view across the different layers, we can also composed it by data producers, data services providers, and data consumer sub-systems which can be operated by different organizations~\cite{ref13}.
%This was accomplished because of efforts and initiatives fostered by regional and international organizations, bringing incentives in the scope of the open government, open science, and FAIR (Findable Accessible Interoperable and Reusable) data principles.

With the increased automation of processes needed due to the increased volume of marine in situ data being collected by marine systems that deal with (near) real-time data streams and the importance of this type of data in the decision-making processes in the domains' industries, it becomes imperial to include data quality concerns by design, ensuring that decisions are made on adequate data. Moreover, the recent incorporation of automated decision-making components based on available new AI solutions~\cite{10188681} that rely on data that can be provided by external systems reinforces the need to understand data quality, which influences the trustworthiness of these systems' output. Similarly, previous studies have discussed the need to investigate the impact of data quality on machine learning and other AI-dependent systems' design~\cite{9609199,kuwajima2020engineering}.
%QA importance at software level - migration to data-driven with automated decision-making based on data, and thus data quality starts to have more impact on the overall systems.
%"Gaps exist in particular for addressing data quality and its design consequences, which is essential in ML systems." 
%https://link.springer.com/article/10.1007/s10994-020-05872-w?code=2c0c0228-4ff9-45e6-9285-d6dace01edc0
Moreover, the European Union (EU) has made significant efforts towards regulating the usage of low-quality data in applications that could potentially impede citizens' rights. The regulatory framework proposal on artificial intelligence\footnote{\href{https://ec.europa.eu/newsroom/dae/redirection/document/75788}{https://ec.europa.eu/newsroom/dae/redirection/document/75788}} aims to ensure that high-risk AI systems adhere to these standards to establish their trustworthiness. While these data-related concerns and requirements are currently not mandatory in ocean-related sectors, initiatives like this one confirm the growing concern about understanding the quality of data. This understanding can help make informed decisions and regulate the oceans. %usage of 

%DQ attributes - combining with existing knowledge on software QAs enabling a more complete analysis of what has become data-driven applications.
With the transition to these complex and ``intelligent'' systems greatly dependent on data, knowledge of their software architecture is crucial to understanding their different layers, the interactions, and the behavior of associated components. The architecture also serves as an abstraction of the system that aims to represent its more significant parts as a means to perform validation or verification, assuring the quality of the system. 
Architectural knowledge and their documentation are crucial for understanding the rationale that must be implemented in its components behavior. The documentation of this knowledge is also important in the maintenance, analysis and evolution of the architecture for understanding the trade-offs and assumptions made when architectural decisions were made~\cite{bass2003software}. Moreover, one of the reasons behind architectural knowledge is the analysis of quality attributes to provide some guarantees over the system.

In this work, we describe a data-flow oriented software architecture developed in an R\&D setting that involves stakeholders with different data-related roles within the marine domain. This ongoing iterative process is a result of a three-year work that incorporated knowledge from the domain present in literature, stakeholders' needs and goals, and integrated stakeholders' legacy systems. 
The process was guided by constraints present in domain-specific challenges where the resources and capabilities grow over the data delivery chain, as in many other IoT systems. Despite that, there is some complexity imposed by the difficulty in re-configuration and maintenance of existing equipment in marine systems that are operated remotely. Moreover, we built our architecture on the analysis of existing domain-specific challenges impacting the software and data quality attributes in the architecture of systems in this context. Lastly, it is important to mention that our research addresses data driven IoUT-enabled systems that are fixed, not considering implications of mobility of nodes inside the UWSN. %assumption
Our aim is to aid practitioners in the marine domain in making the best-informed decisions when architecting their systems by describing architectural decisions that address the major stakeholders' concerns and challenges in the domain. Furthermore, our proposed architectural decisions incorporate software quality attributes, and data quality attributes concerns. We hope to contribute to software architecture research, bringing more studies to the intersection of these topics.
%for stationary remote systems with scarce resources and unreliable wireless communications constraints in other domains of application.

%\keila{Add definition of marine in situ data to address Thanh's comment that generates near real-time data streams.}
%limited battery span, costly (re)deployment and maintenance, and unreliable wireless communications.
%producing data in heterogenous formats that operates in environmental and defense sensitive locations.

The rest of the paper is structured as follows: in section~\ref{sec:method}, we describe the research methodology process followed by the challenges analysis in
in section~\ref{sec:challenges}. After that, we describe the architectural decisions and the resulting architecture in section~\ref{sec:decisions}, followed by the architecture implementation in our context in section~\ref{sec:prototype_arch}. Next, we present some related work in section~\ref{sec:related_work} and discuss our results w.r.t the data flows in section~\ref{sec:discussion}. Finally, we conclude the paper and discuss future work in section~\ref{sec:conclusion}.

%The architecture description is then complemented by the connectors description in Section~\ref{sec:discussion} as a result of the flexibility imposed by the integration of systems developed and operated by different organizations.
%Moreover, the resulting architecture and its implementation in a prototype being built in the context described in Section~\ref{sec:method} are also described in Section~\ref{sec:prototype_arch}.

%\keila{Also introduce IoUT, UWSN, and QAs in general}.

%\input{sections/background}
%\input{sections/method}

\input{sections/method_Thanh}

\input{sections/validity}

\input{sections/challenges}

%\input{sections/results}

\input{sections/decisions}

\input{sections/arch_in_context}

\input{sections/related_work}

\input{sections/discussion}



==> sections/archive/method.tex <==
\section{Methodology}
\label{sec:method}
In this paper, we present a long-term empirical software architecture development process in a cross-organizational setting. This ongoing process has been led by the systems' challenges encountered throughout the different layers of the architecture, imposed by an environment characterized by the limited resources where some of the constituent systems operate and where the data is generated. On the other hand, we have also concerns elicited from regular discussions held in \textit{stakeholders workshops} of the overall system. All these data served as inputs in the process \textit{workflow} summarized in Figure~\ref{fig:method}.

% \begin{figure}[htb!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/icsa_method_round.pdf}
%     \caption{Methodology overview}
%     \label{fig:method}
% \end{figure}
%\thanh{I don't understand the bi-directional arrows between stakeholders workshops and software-related stakeholder workshops, and software-related stakeholder workshops and architect team. Those arrows indicate that the parties validate the ideas of each other, which I don't really think so. Maybe just unidirectional arrows from the top to the bottom?} \keila{I have updated the figure to add feedback and described in the methodology how this feedback is incorporated into a new cycle in the overall workflow process.}

\begin{figure}[h!] % [H] forces the figure to be placed exactly where it appears in the text
	\centering % Horizontally center the figure
	\begin{subfigure}{\linewidth}
    	\centering % Horizontally center the figure
    	\includegraphics[trim={1.5cm 2cm 1.6cm 2cm},clip,width=\linewidth]{figures/method/relevance_cycle_arch.pdf}
        \caption{Relevance Cycle}
        \label{fig:method_relevance}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.6\linewidth}
    	\centering % Horizontally center the figure
     % [trim={left bottom right top},clip]
	\includegraphics[trim={0.5cm 3.5cm 15cm 4.5cm},clip,width=\linewidth]{figures/method/design_cycle.pdf}
    \caption{Design Cycle}
    \label{fig:method_design}
	\end{subfigure}
    \hfill
    \begin{subfigure}{0.3\linewidth}
    	\centering % Horizontally center the figure
     % [trim={left bottom right top},clip]
	\includegraphics[trim={0.5cm 9.5cm 18.5cm 0cm},clip,width=\linewidth]{figures/method/method_legend.pdf}
	\end{subfigure}
	\caption{Design science framework methodology cycles.}
 %\keila{action: - Some figures are too small to be readable (e.g., Fig. 8).}
	\label{Design science framework methodology stages}
    \vspace{-0.2cm}
\end{figure}

Firstly, during spring and autumn every year since 2022, all stakeholders are brought together in a 2-days seminar to discuss the latest advances and on the prototype which includes discussion on the hardware, software and telecommunication parts of the overall system. During these two days, there is also dedicated space to discuss each one of the parts of the system in depth.

Secondly, the monthly workshops conducted with the \textit{software-related stakeholders} fostered more technical discussions with representatives responsible for the systems involved in the data value chain. These representatives come from the organizations listed in Table~\ref{tab:partners} which systems and/or data is being integrated in a prototype wireless autonomous stationary marine observing system. In terms of duration, these workshops took around 2 to 2,5 hours. 

Lastly, in the internal team (authors) involved in the software architecture definition, and because the process is research-based, there is also input from literature besides the feedback from the different discussions with the stakeholders described above. In these meetings, the concerns captured from all inputs are translated in architectural decisions that are than implemented in new constituents, or integrated with the existing ones, tuning the  decisions with the feedback from the \textit{prototyping} process.
When the prototype were tested and validated internally, then the \textit{validation} process starts up the stakeholders chain in the two different workshops with the stakeholders and the \textit{feedback} received there triggers a new cycle in the overall methodology process.
In summary, the following major activities where part of the methodology: 
\begin{itemize}
    \item Monthly workshops from the past 3 years from November 2020 to November 2023. % 19
    \item 2-days biannual seminars from Spring 2022 to Autumn 2023. %4
    \item Weekly meetings from January 2022 to November 2023. %many
\end{itemize}
%\keila{Add duration of meetings: 2hours}

The methodology described gives a high-level view of the process in enough detail to understand the research and development chain to the background and results presented in the following sections. Furthermore, activities such as threat analysis with different stakeholders in their integrated systems are also being taken and has aided in understating the boundaries between the different tiers and the data flow between them.
\subsection{Context}
\label{sec:context}
The work presented in this paper is a result of an ongoing long-term research process to design and prototype the next generation of wireless autonomous stationary marine observing system for different use cases within the domain of application: aquaculture, environment and climate, offshore structure integrity and leakage monitoring. In Table~\ref{tab:partners} we present the organizations with whom the collaboration is being done. All the stakeholders involved in the main three activities conducted throughout the research process belong to these organizations. 
\begin{table}[h]
  %\begin{threeparttable}
  \caption{Organizations involved in the study}\keila{Clarify role, sector, and use cases because of cluster partner. - bring to discussion with Rogardt.}
  \label{tab:partners}
  {\small
  \begin{tabular}{|p{.20cm}|p{.8cm}|p{5.3cm}|p{0.9cm}|}
    %\toprule
    
    %\midrule
    \hline
    \textbf{ID} & \textbf{Size}     & \textbf{Profile }    & \textbf{Role}   \\
       & \textbf{(emp.)} &          &       \\
\hline
    %1       & $<$250    & Physics and technology research group expert in acoustics. & \\
    %\hline % UiB
    1       & $<$250    & Producer of oceanographic sensors and supplier of sensory services & P, S, C\\
    \hline % Metas
    2       & $>$250    & Research institute on technology development for sensors and decision support & C\\
    \hline % NORCE
    3       & $>$250  & Underwater communication and marine robotics manufacturer  &  P, S \\ % Kongsberg
    \hline
    4      & $>$250  & Defence-related research and development institute  &  P, S \\ % FFI
    \hline
    5     & --  & Marine industry cluster to foster technology synergies in the sector &  R  \\
    \hline % GCE OCEAN Tech
    6  & $>$250 & Oil exploration and petroleum resources development company &  C  \\ % AkerBP
    \hline
    7  & $<$250 & Oceanographic sensors manufacturer and sensor services provider &  P, S  \\ % AADI
    \hline
    8     & $<$250  & Manufacturer of underwater communication systems and monitoring services provider &  P, S, C  \\
    \hline % Wsense
    9      & $>$250  & IT and digital solutions consultancy &  S, C  \\
    \hline % Bouvet
    10      & --  & Innovation industry cluster to foster national and international R\&D cooperation &  R  \\
    \hline % GCE NODE
    11     & $<$250    & Research institute focus in marine, cryospheric and atmospheric studies &  P, S, C \\
    %\hline % NERSC
    \hline
    12      & $>$250  & Subsea systems development, operation, and consultancy &  P, S  \\
    \hline % Reach Subsea
    13     & $>$250  & Marine research institute    &  P, S, C \\
    \hline % IMR
    14      & $<$250  & Offshore telecommunications carrier &  S  \\
    \hline % Tampnet
    15     & --  & Cluster of research institutes, governmental bodies, and companies operating within the seafood industry  &  R  \\% Seafood Innovation
    \hline
    16      & $<$250  & Subsea inspection systems development and operation &  P, S  \\
    \hline % TSC Subsea
    %\bottomrule 
\end{tabular}
}
    \begin{tablenotes}
      \item \small
     \hspace{.1cm}
	 P: Data Producer / S: Data Service Provider / C: Data Consumer / R: Representative of stakeholders in a particular sector
    \end{tablenotes}
%\end{threeparttable}
%\vspace{-.5cm}
\end{table}
As for the organizations' roles process for building the overall system, we have divided them into:
\begin{itemize}
    \item Data Producers -- this role comprises organizations that are in charge of developing, integrating, and deploying sensor-based platforms in water. Their system constitutes the Underwater Wireless Sensor Network (UWSN) component of the overall Internet-of-Underwater Things (IoUT). These types of organizations are also responsible for delivering data into the cloud side, creating a bridge from the underneath wireless sensor network layer (edge and fog devices) of typical IoT system architecture.
    \item Data Service Providers -- this role is performed by organizations that provide services throughout the data delivery chain, whether it is telecommunication-related, software-related, or both. These organization does not necessarily need to produce data but in the case of the data producers, they can have services to deliver the data to the cloud side. These services comprise any software system in place that facilitates the transmission, processing, and access to data collected by data producers.
    \item Data Consumers -- On the end user application side, we have organizations that need the data for different purposes in their operations scenarios in the domain of application. These organizations are crucial for the understanding of how the architecture can be parameterized for a specific use case.
    \item Representative -- Some organizations represent groups from the different roles described above, bringing a broader perspective when creating solutions in the different sectors within the domain of application.
\end{itemize}

%\keila{mention ongoing threat analysis sessions}
%\keila{Collect number of WP3 workshops, internal meetings and threat analysis sessions and gather notes from those}


\subsection{Threats to Validity}
% Argue for ad hoc selection of papers for challenges gathering -> domain knowledge gain in the past years
% IoTJ paper references in table 5 and latest papers refering them because since they were surveys there is no point on going on its references
%Many of the Papers are surveys or challenges gathering in venues used by researchers and practicioners in the domain 
% Mention the lack of end user applications on top of the data platform (in the current implementation)

%expertise is perceived as KB in our research methodology paradigm in Hevner
\subsubsection{Construct Validity}

\subsubsection{Internal Validity}

\subsubsection{External Validity}

\subsubsection{Reliability}


==> sections/archive/method_rogardt.tex <==
In this work, we employ the design science paradigm to create the architecture and architectural decisions. Here, we base our approach on Hevner's framework, which consists of three circles: the relevance circle, the rigour circle, and the evaluation circle. First, we will give the context where we conduct our research. 
 
\subsection{Context} %Environment of the research paradigm
We aim to develop the next generation of wireless autonomous stationary marine observing systems for various applications: aquaculture, environmental and climate monitoring, offshore structure integrity assessment, and leakage monitoring. In Table I, we outline the organisations involved in collaboration. These organisations serve three distinct roles:
Data Service Providers: These entities offer services across the data delivery chain, encompassing telecommunication-related and software-related functionalities. While they may not necessarily produce data, in the case of data producers, they provide services to transmit data to the cloud side. These services include software systems facilitating the transmission, processing, and access to data collected by data producers.
Data Consumers: These organisations, situated at the end-user application side, require data for various purposes within their operational scenarios related to the application domain. They play a pivotal role in configuring the architecture for a specific use case.
Representatives: Certain organisations serve as representatives for groups belonging to the aforementioned roles, providing a broader perspective in devising solutions across different sectors within the application domain.
 
\subsection{Relevance Cycle}
Figure A shows that the architecture team involved in this research conducts weekly meetings, each lasting 2 hours. Additionally, we organise monthly software-related workshops where we engage with stakeholders from various areas. These workshops aim to comprehend the software requirements, determine the architecture to develop, identify necessary architectural decisions, and validate our ongoing efforts. Moreover, biannually, we convene the entire consortium. These biannual meetings aim to gain a comprehensive understanding of our software solution within a larger contextual framework.
 
\subsection{Rigor Cycle}
All the architectural challenges discussed in this paper are derived from the references cited ... . These challenges are presented in Figure X. They are primarily deliberated upon during our weekly meetings, where architectural decisions are discussed to address these challenges. Furthermore, these challenges are validated within our monthly workshops.
 
\subsection{Design Cycle} 
In Figure B, you can observe the evaluation process conducted within the architecture team. Architecture decisions are founded upon the identified challenges, leading to the creation of an architecture, followed by the development of a prototype to validate this architecture. Hence, the novelty of this paper lies in the validation of architectural decisions. This validation occurs internally through our iterative process and is further substantiated by discussions during our monthly and biannual meetings.

==> sections/archive/profes22_data_flows.tex <==
\section{Introduction}

In this study, we focus on the intermediate layer between the sensing applications and the smart systems. Inherently, we covered some properties of IoUT in order to understand how to integrate real-time data producers in a data ecosystem.

\section{Background}
There are key technological challenges closely related to the surrounding environment that these systems operates \cite{fattah2020survey,qiu2019underwater}: the limited power supply on the sensing systems, high-associated costs for deployment and maintenance, and limited bandwidth in underwater means topped with costly data packages transmissions from the sensing sites to stations. These challenges limit data available from such systems, which is a key component in understanding and assessing the state of the sensing sites, as well as it is a key component aiding fact-based decision making. As a consequence, not all the data is sent to shore in (near) real-time, leading to an upload of full raw data records only after the instruments undergo an intervention. These practices originate because processing spends fewer resources (energy) than transmission in these cases \cite{qiu2019underwater}, leading to duplication of data that is published, having different levels of processing and quality. 

\subsection{Data Flow}
\label{sec:dataFlow}
Different marine sectors have different demands requiring parametrization. 
These are properties that are configurable by data producers and providers to be able to customize the data received at end-user applications (data consumers) used for decision-making.
In monitoring applications, data in (near) real-time is need because of the resources at stake, either they are the fishes, or offshore infrastructures. The data transmission criticality arises because the purpose of these applications is to expedite the actions to be taken where users are typically interested in anomaly detection in the systems and their causes.  Interviewee subject 11 depicted this critically as follows:
% \begin{quote}
    ``\textit{A lot of users need data right now, and they need to understand if they're going to start feeding or stop feeding, going to port or hold off. For that type of data you may not need as much bandwidth and there's also a different type of speed requirement, in order to fulfill the requirements of the users.
    %They need it right away. I mean they can't look at data from half an hour ago. They need it real-time, so if you're working on dredging and you have turbidity issues where you're you know you're re-suspending a lot sea bottom and you are lowering the oxygen content, you need to stop right away, not after all the fish are dead. So there's a sort of different types of requirements with these different types of usage.
    }''
% \end{quote}

Data outbound properties such as the real-time constraints is also affected by the amount of data that needs to be sent in real-time, which in turn also defines to local processing needs to fit the information needed into the available bandwidth. Interview subject 19, which has a long experience working with the offshore industries explained a requirement imposed by service contractors: 
% \begin{quote}
    ``\textit{...in the requirements for the oil and gas companies that the processing for complex instruments shall happen on the seabed. And then basically only engineering data will be sent to surface like output, not the raw data.}''
% \end{quote}
This property is also verified in other marine fields whose operations relies on surveys such as bathymetry or ocean acoustic tomography and thus the measurements must also be processed heavily to be sent in (near) real-time, or in alternative, it must be retrieved and uploaded upon sensors intervention.

From the implementation side, the goal is to have data received in the second scale, as reported by one of the researchers working in network communications in the underwater and IoT domain (interview subject 2):
% \begin{quote}
%We call it real-time, but it's more near real-time. So 
    ``\textit{Typically it’s from one second to ten seconds after we have done the measurement on the sea, and before we are receiving the data. But for a customer, as long as that (interval) is within one minute then it's OK, so it's not in the millisecond range.}''
% \end{quote}
%Regarding this time dimension of marine data shared, we can have (near) real-time due to the limitations of mostly deployed wireless communications of \textit{in situ} monitoring platforms, or long-term observations and other data products such as forecasts, which can be accessible via web services. This aspect is an influencing factor when it comes to time criticality of the systems for analysis and decision-making. 
% \begin{quote}
    % ``\textit{There's maybe a difference between quick data and slow data analysis and real-time decision making versus looking for bigger trends. You might need raw data you to make aggregated (datasets), or you can look at trends for a long period of time to make a decision.}''
% \end{quote}
%These properties have to be taken into account when sharing data in the marine domain to have enough flexibility to be applied across the different sectors.
Lastly, inbound data flow details are kept out of the study because they are out of scope from the data ecosystem point of view despite being relevant at the IoT level which is managed by the organization producing the data.

\subsection{Quality Attributes}
When it comes to the data availability must be the major component in data-driven systems.
Also related with data availability will be the bandwidth usage optimization, which in other words is captured by the throughput of the \textbf{performance} attribute.
\subsubsection{Trade-offs}
The criticality in terms of time constraints in the ecosystem can be affected whether the information engagement is performed at edge nodes, i.e. closer to the sensors, or at the cloud level since the throughput and latency can improve greatly along the data delivery chain because of the communication technologies used (e.g. acoustic, mobile broadband or satellite, and internet). In contrast, the throughput requirements can also be affected by the reliability in terms of the availability and failure of these communication technologies.  As a result, there must also be a compromise between fault tolerance and throughput requirements.

Another architectural trade-off w.r.t. to have in mind is the resource utilization at the IoUT level. A balance between energy consumption and operations such as data transmission or local processing is taken into account in the autonomous marine systems design. %In our study, we found that computing operations can consume less battery than transmission device operations.

\paragraph{\textbf{Reliability, Usability, and Security \textit{vs} Performance.}}
%\subsubsection{Throughput (Performance) \textit{vs} Transmission constraints (Reliability)} %Trust?
In general, quality attributes closely related to data and its usage can affect negatively the performance of the ecosystem. As previously mentioned, data quality assurance automated procedures can have repercussions on the performance of the overall analytics workflow \cite{dataops}. At the same time,  procedures to enforce the correctness, understandability, and integrity of information exchanged in the ecosystem can also insert more overhead into throughput metrics in the performance.

==> sections/archive/profes22_data_sharing_categories.tex <==
\subsection{Categories of data sharing}
\label{sec:categories}
When it comes to current categories of data sharing in terms of access, we have identified the following:
\begin{itemize}
    \item \textbf{Open-access data} -- Big-data public infrastructures which are responsible for the collection and curation of data from different sectors, making most of them publicly available through some services. Aspects such as standards, conventions, and vocabularies are well established, and are being used at a greater scale by international agencies. An example of this type of platforms is  the Marine Copernicus Service\footnote{\url{https://marine.copernicus.eu/}} which operates at the European level. %Regarding the access control, services such as the marineId is used to register and authenticate data consumers, not only at European level, but also at other major marine data infrastructure such as the NOAA/NCEI big data platform\cite{NOAANCEI}.
    \item \textbf{Restricted data} -- This type of data suffers from various constraints, we have divided them into three sub-categories. 
    \begin{itemize}
        \item \textbf{Legally restricted} -- Data that cannot or has to be shared to compliance with laws and regulations.
        \item \textbf{Business critical} -- Data that contains critical information for business operations, e.g. ''sensitive data''. This type of data is critical not only for data owners (oils companies and such) but also for data providers to improve sensor measurements. These service providers are required to process a lot of data locally because of the bandwidth constraints.
        \item \textbf{Resource depending} -- Data that can cause no harm to sharing entity, e.g. ''non-footprint'',  and can be valuable to a third party entity or to new applications, but requires resources/infrastructures be shared. This data, of is not being sent can be easily overwritten since storage can also be a constraint in the sensing devices or at the edge sensor hubs. %Infrastructure demanding
    \end{itemize}
\end{itemize}
These categories are to be taken into account in the migration to data ecosystems paradigm as some of the characteristics of the domain that needs to be expressed in the system.

==> sections/archive/reliability_performance_energy.tex <==
%\paragraph{Reliability and Performance efficiency}
\subsection{Reliability and Performance Efficiency}
\label{sec:reliability}
\rogardt{Why are Reliability and Performance Efficiency in the same subsection? Are they really related. I do not get the feeling of that?}

Because of the impact of the underwater acoustic signals on marine life, there could be restrictions on the transmission windows and frequencies (\textbf{performance efficiency}). The noise generated by the communication device's signals can negatively impact species that use acoustics to communicate or prey, e.g., by leading them to confusion or causing other changes in the behavior (\textbf{CH6}).
%Concerning \textbf{performance efficiency}, the impact of the underwater acoustic signals on marine life might put restrictions on the transmission windows and frequencies according to the ecosystem surrounding the operations infrastructure at sea. 
This challenge has implications on the communication channels and links utilization (\textbf{resource utilization}). %Furthermore, the noise generated by the communication device's signals can negatively impact species that use acoustics to communicate or prey leading to confusion or other behavior changes (\textbf{CH6}). %As a consequence, this constraint can impact the \textbf{availability} of data.

When it comes to \textbf{reliability} at the underwater data acquisition layer, the only power source for underwater equipment is the battery. This limited resource lifetime can vary from a few weeks to years depending on the data sampling rate, the precision of instruments, and the power consumption of the transmission device (\textbf{CH9}). This last factor is due to the higher consumption of energy associated with transmission devices when compared to computation done locally. Thus, \textbf{energy efficiency} is one of the main drivers of the overall system.\thanh{hard for me to link limited energy to reliability, isn't it still about performance efficiency?}
%This challenge forces software embedded in sensor nodes to optimize power consumption, which includes managing processing and transmission tasks. Regarding these tasks, there are indications that transmission devices consume more energy than computation, and components can be temporarily powered off to save energy (sleep mode)~\cite{ref14}.
Furthermore, at the UWSN level, underwater sensors, communication modems, and gateways are vulnerable to physical impacts. For example, equipments can be damaged by human activities (e.g., hit by ships) or by nature (e.g., dragged by sea waves, currents, or ice). This can affect sensor measurements, device integrity and their resulting data quality. \thanh{it becomes a bit clearer here for reliability, but I agree with Rogardt that there is no link between reliability and performance effienciency.}

In the network communication layer, wireless communication channels in IoUT have less available bandwidth per packet transmission (\textbf{CH7}) compared to traditional land-based channels. This is the case for the acoustics in underwater communications and satellite in over-the-air communication (OTA), where latency can vary according to atmospheric or water conditions (e.g. affected by absorption). These challenges constrain the overall network \textbf{performance efficiency capacity} of software systems in IoUT environments.\thanh{the discussion seems to back and forth. First, it was about performance efficiency, then reliabity, and now performance efficiency again. Would that be possible to link them here? The next paragraph seems to better do the job.} Lastly, the OTA options (satellite and mobile networks) to transmit data into IP networks usually have higher costs associated with the carrier service.

In summary, while the physical vulnerability (\textbf{CH2}) of the hardware and the limited battery (\textbf{CH1}) affects the availability of the software system (its operation), the unreliability associated with the wireless underwater network links (\textbf{CH4}) impacts the capacity of the software system to operate in the presence of faults in the communication channel. %recoverability implication as well 
\rogardt{What do recoverability have to do with Reliability and Performance Efficiency?}
Overall, these challenges impact the \textbf{recoverability} data quality attribute, i.e., its ``\textit{degree to which data has attributes that enable it to maintain and preserve a specified level of operations and quality, even in the event of failure}''~\cite{iso25012}.
%Moreover, the power-demanding UAC transmissions (\textbf{CH9}) is a failure which could impact data availability.  %\paragraph{Energy efficiency}
%Transmissions must be handled carefully to avoid the drainage of the battery power because communication devices can be the component that consumes more energy in the systems at the UWSN level. 
%As pointed out in~\cite{bass2003software}, \textbf{energy efficiency} of software systems can no longer be disregarded.
%In the marine domain, \textbf{energy efficiency} is one of the main drivers of the overall system because of its implication on the availability of the systems and the data produced by them due to the risk of power down and the time and costs to its maintenance.\lars{This last sentence appears a bit otu of context for me - it is a bit forth and back?} % (e.g. battery replacement operations).

==> sections/archive/results.tex <==
\section{Data-flow oriented Software Architecture}
\label{sec:results}
In this section, we describe in detail the architectural decisions that resulted from the process described in Section~\ref{sec:method}. All the decisions, which were summarized in Table~\ref{tab:decisiosn}, are made with the challenges presented in the previous section in mind and thus aid in mitigating the quality attributes affected by those. When making the architectural decisions, the challenges are not addressed in isolation but instead in context with other challenges, conflicting or related challenges, the stakeholders' needs and feedback, and incorporating with the existing architecture for integration with existing and legacy components and systems. Throughout the description of architectural decisions, we also explain how those appear in the resulting architecture layout in the overview in Figure~\ref{fig:arch}. The architecture description is then complemented by the connectors description in Section~\ref{sec:flows} as a result of the flexibility imposed by the integration of systems developed and operated by different organizations.
Moreover, the resulting architecture and its implementation in a prototype being built in the context described in Section~\ref{sec:method} are also described in Section~\ref{sec:prototype_arch}.

\subsection{Architectural Decisions}
\label{sec:decisions}
In this section, we describe in detail the rationale behind the architectural decisions made to address the challenges listed in Table~\ref{tab:challenges}.
Architectural decisions describe the rationale, risks, and assumptions made during the design process of a software system. This description is crucial not only for the implementation stage but also for the analysis of the architecture, especially in its maintenance~\cite{bass2003software}. %trade-offs as well

\paragraph{Distributed data processing and transmission (AD1)}
%Assumption: data is considered the measurement value (after signal conversion - output of sensor)
%When migrating, building, or deploying a system for real-time in situ marine data acquisition and sharing in a cross-organizational context, 
%These constrains boils down to a optimization problem between the amount of data to be sent, the transmission rate
%influences the sampling rate?
%also addressing the quality attributes affected by the specificity introduced by the challenges at the first two layer of the overall system:
% \begin{itemize}
%     \item Volume, resolution, and throughput of data
%     \item Environmental impact of communication + number of devices
% \end{itemize}
%Depends on the configuration, deployed capability, and operational scenario requirements:
%Should have the possibility to send only "data diffs" (changes in data) -  tradeoff between energy efficiency, data availability and volume (compression) - reconstruct information if needed* - reduce impact on the environment
%One should consider the following concerns regarding the configuration of the software components involved in the data acquisition and the data delivery chain to meet the operational scenarios. These components can help address the challenges associated with data acquisition and network communication, which constraints impose tradeoffs on the resulting software architecture. 
There are many concerns to be balanced when implementing the components in the data acquisition and network communication layers, in order to meet the operational scenarios requirements.
More specifically, there is a tradeoff among the volume of data sent, the power consumption to transmit data (challenge \textbf{CH9}) in the UWSN, and the density of the wireless communicating nodes in the area to cover and their impacts when transmitting data wirelessly (challenges \textbf{CH6}). On the one hand, the volume of data depends on the number of sensor devices deployed, their configured sampling rate, security mitigation strategies (challenge CH8), and the power consumption in the nodes inside the UWSN (challenge \textbf{CH1}). These aspects are part of the responsibilities of the \texttt{Sensor} component in the overall architecture layout in Figure~\ref{fig:arch}.
On the other hand, the available bandwidth and latency can vary with the water's physical properties being in best conditions already very limited when compared to the amount of data that can be generated or the bandwidth available in typical land-based systems, creating a bottleneck in the throughput (challenges \textbf{CH4} and \textbf{CH7}). Lastly, each transmitted message inside the
UWSN can impact the life and the surrounding ecosystem. This decision reflects the systems' environment, bringing computation closer to data acquisition instead of sending raw data to be processed on the cloud level where more resources are available (challenge \textbf{CH5}). The \texttt{Local Processing} component in the resulting architecture depicted in Figure~\ref{fig:arch} is a consequence of this, being
responsible for aggregating and fusing raw measurement data from the different sensors in UWSN. Local computation is associated with the transmission of data because of the limited wireless communication options and the unfeasibility and cost of employing wired communications from sea to shore. When it comes to the transport inside the UWSN, \textit{ad hoc} protocols are needed when transmitting data between the different nodes until the surface gateway. There is also a need to serialize the data for the different communication channels and devices. This behavior is part of the responsibilities of the \texttt{Communication Management} component depicted in Figure~\ref{fig:arch}, which is also responsible for bridging data between different physical channels, e.g., underwater acoustics and over-the-air technologies. In turn, the surface gateways have to bridge to long-range transmission channels provided by satellite links or mobile networks (e.g. 4G or 5G) using the carriers' standardized APIs.


\paragraph{Data Platform (AD2)} To address the interoperability issue introduced by challenge \textbf{CH12}, there was a decision to have a data platform built to allow data aggregation from different sources before its usage on the application level in the different use cases within the marine domain. The rationale behind this decision was to have a common configurable platform that can be parametrized when interfacing with the other layers according to its operational scenario requirements. Although some processing is done in the lowest layers, at the platform level, data fusion is performed, aggregating data from different sensing platforms. Thus, it is assumed that the volume of data is greater at this level despite sharing the property of dealing with heterogeneous data formats at device and data source ingestion, accordingly. In the resulting architecture presented in Figure~\ref{fig:arch}, this decision is reflected in the \texttt{Ingested Data
Processing}, the \texttt{DBMS}, and the \texttt{Access Control} components on the right side.
%
\paragraph{Message-oriented data ingestion middleware (AD3)}
Message-oriented data ingestion middleware (AD3): The rationale for this decision was to use a standardized way to provide data that is delivered by different (distributed) systems to \texttt{Data Consumer Application}s. By using the publish-subscribe pattern, we decouple data-producing systems from data-consumer systems, bringing more flexibility when handling outages from each one of these types of systems. With this pattern, data producers and consumers do not need to know or keep information about each other, transferring the responsibilities to a broker component that can also handle concurrent data ingestion and provisions to the different systems that might connect to it over time. The resulting architecture presented in Figure~\ref{fig:arch} implements this component via the Ingestion Broker. This decision adapts to the uncertainty introduced by unreliable communications and the physical vulnerability of the components in the underwater data acquisition and the network communication layers (challenges \textbf{CH1}, \textbf{CH2}, and \textbf{CH9}), affecting data reliability and availability of data, on the software and system-dependent data quality side respectively.
%
\paragraph{MQTT Protocol (AD4)} MQTT is an OASIS standard protocol for message exchange in IoT-enabled systems and it is used on the top of the publish-subscribe communication model pattern. Its lightweight (low footprint and small message size) characteristic and simplicity in implementation has fomented a creation of large community and services built on top of the protocol~\cite{mqtt_survey}. Another important characteristics of the protocol are the definition Quality-of-Service (QoS) levels\footnote{The QoS levels are applied to the sender and receiver of the message (publisher-broker or broker-subscriber), and thus the end-to-end quality of service level must be implemented on the top of the protocol usage.}:
\begin{itemize}
    \item At most once (level 0) -- should be used in operational scenarios that data loss is permitted.
    \item At least once (level 1) -- should be used in operational scenarios that duplicated data delivery is permitted.
    \item Exactly once (level 2) -- should be used in operational scenarios that requires assure of data delivery without duplicates.
\end{itemize} 
Depending on the network protocol inside the UWSN which defines the behaviour for re-transmissions for the surface gateway systems, it might be more adequate to deploy the different QoS levels from the communication between the \texttt{Surface Gateway} and the \texttt{Ingestion Broker} component, and addressing the uncertainty introduced by the unreliable underwater wireless communication (\textbf{CH4}).
The low footprint also fits well to the low communication bandwidth and high operation costs of satellite link (challenge \textbf{CH7}), and contributes with its low overhead to save bandwidth and potentially the number of transmissions needed (challenge \textbf{CH9}).
These characteristics were behind the selection of the protocol for the transmission of data from the different data producers' devices at sea, and into the data platform. Furthermore, the size of the data to be transmitted was also took into consideration for the selection of a suitable network protocol solution.

\paragraph{Platform monitoring (AD5)}
The main driver for this decision was the different causes of faults that impact the layers inside the UWSN, affecting the availability of data on the \texttt{Ingested Data Processing} component. Since there is a runtime dependency of the system behavior on data, it is crucial to detect errors that occur in runtime as early as possible to trigger context information for root cause analysis and shorten the recoverability of the overall system. More specifically, it addresses the challenges at the data acquisition and network layers,  causing uncertainty in the data availability introduced by unreliable communication, physical vulnerability, and limited battery (challenges \textbf{CH1}, \textbf{CH2}, and \textbf{CH4}).
This decision also encompasses the monitoring of the interactions of the data platform with the external systems. Not only the ingestion of data (challenge \textbf{CH12}) but also the consumption of data to help access the usage of the overall data management layers components to provide data to the rightful consumer applications systems (challenges \textbf{CH13} and \textbf{CH15}). For this decision to be implemented, components and data instrumentation, i.e., measurement and recording of their runtime outputted behavior, are needed. Thus, intervention in the different parts of the architecture is required, becoming a cross-cutting concern.

\paragraph{Data Quality Control (AD6)}
Data quality is one of the main drivers and concerns of all stakeholders across the different organizations. It is reflected in challenge \textbf{CH11}, and understanding it for the various marine use cases is crucial for trusting the decisions made on the provided data. In this domain, because of the restricted wireless underwater communication, there is an additional level of complexity when trying to understand the quality of data because of the small volume of data that can be ingested into the data management layer (challenge \textbf{CH5}). Knowledge about the UWSN must be kept and updated to be used during the quality control process, and this task can be distributed across the
different processing components (\texttt{Local Processing} and \texttt{Stream Processing}) layout in the overall architecture depicted in Figure~\ref{fig:arch}.  In particular, metadata information about the measurement systems (sensors) is needed to understand the level of quality of data and its suitability for a specific use case. Additional contextual metadata information recorded throughout the data delivery pipeline (\texttt{Monitoring}) and other related historical data sources might be used to assess and ensure the quality of the data on the real-time data streams. Furthermore, the different data source format standards (challenge \textbf{CH12}) also affect the understanding of data adequacy according to the available information contained in the format for its use in the context of the different use cases.

%This decision reflects in the \texttt{Stream Processing} component at the data management layer in the overall architecture layout in Figure~\ref{fig:arch}.
\paragraph{Data model for integrated data sources (AD7)}   
 On one hand, as a result of the \texttt{Local Processing}, there is a resulting data source in a proprietary format for each organization that is then integrated for the different \texttt{Data Consumer Application}s. The integration is needed because data producers have to incorporate sensors manufactured by others and deal with different device output formats (challenge \textbf{CH3}). On the other hand, as a consequence of the diverse data formats and standards used to ingest data from the UWSN (challenge CH12), there was a need to have a uniform format for the processing done by the different services inside the \texttt{Stream Processing}, simplifying the development of the services upon a single format, addressing and fostering a single understanding of the data at the data management layer. This decision aims to create a representative and flexible model to provide an adequate level of understanding (metadata) of data and its quality, addressing the challenges of the understandability of data for the different use cases (challenge \textbf{CH10}). However, a challenge introduced by this decision is handling the model evolution as required information and available fields change over time and keeping backward compatibility to expected formats on the \texttt{Data Consumer Application} side.

\paragraph{Identity provider (AD8)}
For the ingestion and sharing of the data in the data platform, there must be mechanisms to verify the identity of the systems interacting. There is also a need to ensure correct access, which can only be managed by knowing the identity of the systems. Being the data platform the intermediary component with knowledge about data producers and \texttt{Data Consumer Application}s, it can be used in the management of access to the data streams, addressing the access control challenge (challenge \textbf{CH15}) on the one hand and establishing a baseline for the selective process of sharing of data either it is sensitive (challenge \textbf{CH13}) or not.
During the integration of the systems from the various organizations, there was also an interoperability issue among the different authentication methods and solutions. The rationale behind this decision was to unify the authentication of components and their associated authorization to the different ingested and sharing flows of data. Additionally, since various frameworks can be deployed between the decoupled high-level components in the architecture presented in Figure~\ref{fig:arch}, especially for the ones at the cloud level, the authentication solutions provided by those must also be integrated.
Therefore, this is a fundamental and cross-cutting concern for the interactions between the different components.


\paragraph{Data sharing access control (AD9)}
When data is delivered to the \texttt{Data Consumer Application} component, there is a need for mechanisms to authorize access to the different flows of data (challenge \textbf{CH15}) according to the data category and its degree of ``openness''. This decision helps address challenges in accessing or vetting sensitive
data (challenge \textbf{CH13}) and managing the ingestion into the \texttt{Data Consumer Application}'s side because of the reusability challenge (challenge \textbf{CH14}). This decision depends on an identity solution for the interacting systems and thus is closely related to the previous one (AD8), and together, they constitute a cross-cutting concern regarding ensuring security at the data management layer. 
%Because of the reusability introduced by challenge CH15, not all data can simply be forward to the \texttt{Data Consumer Application}, and thus
This decision’s behavior is implemented via the \texttt{Access Control} component presented in the architecture overview in Figure~\ref{fig:arch}. This component must impose the rules defined at the authentication and authorization management, integrating with the various ways to deliver data via the \texttt{Core Broker} and the \texttt{DBMS} using the push and pull methods to the \texttt{Data Consumer Application}. 

\paragraph{Data classification and triage (AD10)}
Complementary to the access control decision (AD9), an intermediary step is needed to classify the ingested data streams. One of the major drivers behind this decision is the sensitive data (challenge \textbf{CH13}) because of its reusability (challenge \textbf{CH14}) in a context different from the one for which the data acquisition was designed. The rationale for this decision is to filter different categories, quality levels, and ``openness'' of data impacting the \texttt{Access Control} to data shared on the \texttt{Data Consumer Application} components. In the resulting architecture depicted in Figure~\ref{fig:arch}, the \texttt{Stream Processing} component is responsible for implementing the behavior behind the rationale of this decision.


%\keila{Add column impact: cross-organizational or inter-organizational (i.e., data provider, data producer, service/platform provider)}
\begin{table}[hbt!]
\caption{Summary of Architectural Decisions}
\label{tab:decisiosn}
\centering
\scriptsize
{
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Architectural Decision}} & \multicolumn{1}{c|}{\textbf{Challenges}} \\ \hline
AD1 & \begin{tabular}[c]{@{}l@{}}Distributed data processing and transmission\\  responsabilities\end{tabular} & \begin{tabular}[c]{@{}l@{}}CH1, CH4, CH5, CH6, \\ CH7, CH8 CH9\end{tabular}  \\ \hline
AD2 & Data platform & CH12 \\ \hline
AD3 & \begin{tabular}[c]{@{}l@{}}Message oriented data ingestion middleware\end{tabular} & \begin{tabular}[c]{@{}l@{}}CH1, CH2, CH9\end{tabular}  \\ \hline
AD4 & MQTT messaging protocol & \begin{tabular}[c]{@{}l@{}}CH4, CH7, CH9\end{tabular}  \\ \hline
AD5 & Platform monitoring & \begin{tabular}[c]{@{}l@{}}CH1, CH2, CH4, CH12,\\CH13, CH15\end{tabular}  \\ \hline
AD6 & Data quality control & \begin{tabular}[c]{@{}l@{}}CH5, CH11, CH12\end{tabular}  \\ \hline
AD7 & Data model for integrated data sources & \begin{tabular}[c]{@{}l@{}}CH3, CH10, CH12\end{tabular}  \\ \hline
AD8 & Identity provider & CH13, CH15  \\ \hline
AD9 & Data sharing access control& \begin{tabular}[c]{@{}l@{}}CH13, CH14\\ CH15\end{tabular} \\ \hline
AD10 & Data classification and triage & CH13, CH14  \\ \hline
\end{tabular}
}
\end{table}




\subsection{Data Flows}
\label{sec:flows}
% Governance implications - conflicts in PROFES'22 paper
In this section we describe the different flows of data, complementing the description of the components done in Section~\ref{sec:decisions} in the overall software architecture depicted in Figure~\ref{fig:arch}. 

\begin{figure*}[htb!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/arch_overview.pdf}
    \caption{Overview of the resulting architecture.} %Component-and-connector 
    \label{fig:arch}
\end{figure*}
%\thanh{Would be better to use different notations for component and cross-cutting concern. It is difficult to distinguish them. Also, try to have the texts and drawings in black. If you do not change anything, it would be gray as the default option of Google Presentation.}

\subsubsection{Organizational Data Flow}
\label{sec:org_flow}
%\paragraph{Underwater Wireless Sensor Network (UWSN)}
At the Underwater Wireless Sensor Network (UWSN) level, concerning the sensing, processing, and surface nodes in the edge, those are managed by the organization that developed and deployed them as a service. These systems are responsible for delivering data further up until the decision-making side at the \texttt{Data Consumer Application}s. 
Because of the custom hardware setup of the data producers’ managed systems, the data can flow among the processing and transmitting components, traversing different traces according to the routing protocols inside the UWSN. From the point of view of the data delivery chain, the components at this level must optimize the data to be sent up, prioritizing what is more relevant for the operations in case
there are conflicts in the bandwidth usage. At the same time, there is a trade-off to this to balance the battery and environmental impact of the data delivery in (near) real-time (architectural decision AD1). 

Regarding the cross-cutting concerns, on the one hand, the data producer systems are able to remotely monitor and configure the nodes inside the UWSN. To implement this behavior, local agents are also needed to collect information on the nodes state and to interpret the commands coming from control stations in the opposite direction of the marine data flow delivery. On the other hand, concerning the security inside of the UWSN, there are no domain-specific solutions to address the challenge of securing underwater wireless communications in the case of obstruction of the communication channels (denial-of-service), or a compromised node (spoofing) since the update of deployed node is not a trivial task. Solutions used on other wireless communication and IP networks can be deployed but the constraints of the systems' operation in this context must be taken into account. Furthermore, the likelihood of attacks should also be considered in the risk assessment when specifying the requirements according to the degree of ``sensitivity'' of data being collected and transmitted at the UWSN level.
%\paragraph{Cloud} 
% ingested data sources processing -> deliver everything in the same format by the end of the processing pipeline - common understanding from heterogenous data.

At the cloud level, the \texttt{Ingested Data Processing} sub-components are loosely coupled for the elasticity of the computation for the variable volume of data flowing from the different sources pushed or pulled into the pipeline, but also because data might need various processing services according to its quality. The first step into the processing of heterogeneous data streams ingested is to convert it to a complying syntax and semantics at this level, assuring that all the components work upon the same specification and understanding of data (architectural decision AD7). This component also is responsible for validating the ingested data, contributing to the completeness and compliance quality attributes of data. If the storage of data in its raw format is desired for future reprocessing or analysis, this can be achieved by the architecture proposed in Figure~\ref{fig:arch}.

After the \texttt{Data Transformation} process, data is again ingested in a processing pipeline where different services can be invoked. The \texttt{Stream Processing} component is responsible for the data quality control, which will check whether a recently data point is good or bad. The check is triggered once a data point arrives to cope with real-time data usage requirement from data consumers. In case a data point is missing due to, for example, communication issues, sensor faults, the component generates a missing value and triggers an alarm. The quality of data is assessed by four data quality attributes as introduced in Section~\ref{sec:intrinsics_QA}. To perform data quality control in real-time, additional information might be need not only from the measurement side (UWSN) but also from historical data around the same location or from marine phenomenon. Another responsibility held by this component is the categorization for sharing enabling the enforcement of the access control rules.\keila{explain the relation to the stream processing}
%\thanh{Seems irrelevant, suggest to remove.}\keila{This is related with AD10}\thanh{I guess you want to keep it?}

Lastly, when it comes to the storage of the incoming data, the data model will be have a great impact into the selection of solutions for the database management system (\texttt{DBMS} component in Figure~\ref{fig:arch}). With the increase of data volume caused by the deployment or additional sensing platforms, and with changes in the data requirements overtime from the \texttt{Data Consumer Application}, it is important to have a flexible database model to minimize the overload when updating the components with the evolution of the data model fields requirements.

\subsubsection{Cross-Organizational Data Flow}
\label{sec:cross_flow}
To enable the flexibility on the delivery of data to the cloud side, there are three traces for data ingestion in the \texttt{Ingested Data Processing} component. In the proposed architecture, this can be achieved via:
\begin{itemize} 
    \item \texttt{Data Pusher} -- this component is responsible to integrate data sources at the cloud level interacting with data producers' systems over IP networks. In this case of data ingestion, the responsibility lays on the data producers side to push data into the \texttt{Ingested Data Processing} high-level component.
    \item \texttt{Data Fetcher} -- another way to ingest data into the \texttt{Ingested Data Processing} high-level component, is through the component that behaves as a fetcher pulling data from ephemeral data acquisition systems (manual/ship sea surveys), at rest from other accessible databases, or from other streams into the processing pipeline.
    %\texttt{Historical Data Fetcher} -- pulls data from ephemeral data acquisition systems (manual/ship surveys) or from data at rest in other accessible databases.
    \item \texttt{Edge Integration Management} -- this component differs from the other on its physical location at the UWSN level. By using this component, the data sources integration is performed closer to the data acquisition, with more access to information this layer. For this component to be implemented the data acquisition layer has to be exposed for integration with external system in the point of view of the organization operating the sensing platforms.
\end{itemize}
The existence of neither of the components described above are exclusive, this is a reflection of the distribution of processing and communication responsibilities encompassed in the first architectural decision (see AD1 in Table~\ref{tab:decisiosn}). 
Furthermore, in the next section we explain how two of them are currently implemented in practice in this context.

Finally, on the cross-organizational data flow between the data management layer and the \texttt{Data Consumer Application}, there is a need to make heterogeneous components authentication methods uniform to assure the enforcement of the sharing rules and policies to operations and decision-making systems, regulatory data delivery, or data reusability in open-data platforms. This component is also needed to regulate the access to data with push and pull methods (from the \texttt{Core Broker} or the \texttt{DBMS} respectively), in similarity to the ingestion of that into this data management layer. Those rules and policies are implemented via the \texttt{Access Control} component.

\subsection{Architecture in Context} %Prototype implementation architecture
\label{sec:prototype_arch}

\begin{figure*}[htb!]
    \centering
    \includegraphics[trim={1.4cm 0cm 0cm 0cm},clip,width=0.7\linewidth]{figures/prototype_with_tiers.pdf}
    \caption{Overview of the architecture in the prototype implementation.}
    \label{fig:prototype}
\end{figure*}

The prototype implementation presented in Figure~\ref{fig:prototype} reflects the ongoing migration process to the proposed architecture described throughout the previous sections. Many factors come into play for the realization of this migration, making it a complex and slow process. More specifically, the cross-organizational dependency for the development and operation of different block of components in overall architecture. %Secondly,  
%range checks - knowledge on the sensors - calibration and precision of measurements info
%tiers -  Hybrid cloud computing - explain figure legend - some are phisical machines other can be virtual machines since cloud resources computing services are used.

In the prototype there are currently two data producers organizations with different data acquisition and network communication setups, as we can see in Figure~\ref{fig:prototype}:
\begin{itemize}
    \item Organization 7 has in his portfolio a vertically integrated sensor (physical) platform that incorporates all the needed components for the data acquisition and network layers. There are currently two of these platforms deployed at sea and sending data approximately every 30 minutes to their control and storage platform.
    While this setup avoids the use of wireless underwater communication, it also presents a single point of failure and needs to be combined with the deployment of other platforms to expand the area coverage.
    \item Organization 8 has a more flexible setup, with a mesh of nodes distributed among the same area of interest and with adaptive roles locally coordinated by their gateway at the edge of the UWSN. There are currently two sensing nodes and one gateway sending data to their data platform approximately every hour.
    %By having underwater wireless communication between the different nodes (sensing nodes and the surface gateway), there is also a need to secure this interaction as a result of challenge CH9 (see Table~\ref{tab:challenges}).
\end{itemize}
Both organizations are using mobile networks to transmit data over-the-air to their data platform, using the \texttt{Network Carrier
Gateway} component.

For the security inside the UWSN, because of the flexibility and distribution of components, there might be no wireless underwater data transmission and thus, the challenge \textbf{CH9} (see Table~\ref{tab:challenges}) associated with that link does not apply. This is the case for organization's 7 system's components architecture, employs all the needed components in the same physical system with serial or ethernet connections from the sensors to the surface gateway. On the other hand,  there could also be a mesh of nodes physically distributed, which the case of the configuration of the system for organization 8. The security inside their UWSN is provided by tailored framework that follows the NIST recommended levels of security in~\cite{nist_csf} with the focus on low overhead in the underwater communications.

%"The WMesh includes a security framework that implements encryption algorithms and digital signatures enabling the confidentiality, integrity, authentication and non-repudiation. The security framework has been designed to be tailored for the underwater communication allowing the security level recommended by the NIST with a really low overhead in the communication."

At the cloud level, the authors associated organization is responsible for the implementation of the components at the data management layer for the heterogeneous data streams ingested by the data producers' systems. The implemented \texttt{Ingested Data Processing} component is currently transforming, quality controlling, and forwarding data sources ingested in JSON and XML formats by the different data producers.
For the cross-organizational integration done at the cloud level, and as a consequence of the message-oriented middleware for data ingestion (AD3), provoked the development of a new way of delivering data for the existing data platform of organizations 7 and 8 (see Table~\ref{tab:partners}). These changes were  done to implement the expected behavior for the \texttt{Data Pusher} component of the overall architecture presented in Figure~\ref{fig:arch}, and receiving the data as soon as it arrives on the different clouds. While for organization 7 all the efforts where done on their side to complete the migration process, in the organization 8 data integration using the push behavior, the \texttt{Data Pusher} component was implemented on the data management side to bridge the data provided via their own MQTT broker. Lastly, regading data ingestion, since the data was initially povided by organization 8 via a REST API using the \texttt{Data Fetcher} component, this ingestion method can still be used to retrieve historical data or in case of down time (availability issues) on the sending or receiving components. 

For the \texttt{Monitoring} component, we are monitoring Key Performance Indicators (KPI) for the data platform. These KPIs function as service level objectives and are translated to interact with the Prometheus  monitoring toolkit where runtime metrics are stored~\footnote{\url{https://prometheus.io/}}.

Concerning the data provision to \texttt{Data Consumer Application}s, the currently prototype is dealing with heterogeneous authentication methods challenge being in the process of migrating to a centralized authentication  method using the keycloak~\footnote{\url{https://www.keycloak.org/}} identity and access management solution to enable the implementation of the \texttt{Access Control} component. 
%Nevertheless, for testing proposes, a \texttt{Data Consumer Application} has being integrated to visualize the data coming from the different streams. A public version of this integration with a virtual sensor stream is available in: \url{https://thingspeak.com/channels/2129424}.\thanh{The channel location shows Bergen. In Section~\ref{sec:method}, we say~\cite{ref14}, which is our IoT paper, is the starting point of our study. Would that be dangerous that the reviewers discover who we are as they can find out the authors of~\cite{ref14} are from Bergen? Would they blame us that we do not comply with the double-blind review policy?}
Lastly on the \texttt{Data Consumer Application}s side, efforts are being made to deliver data to a data visualization and analytics software operated by organization 2, and to a marine data archive managed by organization 13 (see Table~\ref{tab:partners}). To accomplish this milestone, the data classification must also be performed in the \texttt{Stream Processing} component.

%solutions when it comes to the automation of distributibution and update of credencial in a cross-organizational context


==> sections/background.tex <==
\section{Background}
\label{sec:background}
In this section we introduce software and data products quality attributes from standardized models in section~\ref{sec:challenges}. Moreover, since these standards models are not able to capture all the impacting concerns from the the identified challenges, additional quality attributes form literature are adopted for the purpose. \keila{Also introduce IoUT, UWSN, and QAs in general}.
%Lastly, in sections~\ref{sec:system_QA} and~\ref{sec:intrinsics_QA}, we describe main quality attributes negatively impacted by the identified challenges, describing their effect on the resulting software architecture.
%\subsection{Quality Attributes for Software and Data}
%\label{sec:QA}

%\keila{Discuss the need for the data quality attribute at the software side or just give N/A as done at the data quality side.}

Because of the system's behavior dependence on data quality, we have analyzed the gathered challenges with regards to quality attributes for software and data products from the ISO/IEC 25010~\cite{iso25010} and the ISO/IEC 25012~\cite{iso25012} quality models respectively. Despite that, there was a need to introduce two more quality attributes on the software quality model for accommodating challenges' concerns not captured by the existing ones. More specifically, we adopted the Energy efficiency suggested in~\cite{bass2003software} and Explainability from~\cite{9609199}. 
While the sustainability of architectural decisions remain an open challenge and relates to the evolution of systems~\cite{VENTERS2018174}, characteristics such systems' energy efficiency~\cite{bass2003software,VENTERS2018174,koccak2015integrating} are identified across different studies as quality attributes to consider when evaluating software systems. Even though the ISO/IEC 25010~\cite{iso25010} encompasses a resource utilization sub-characteristic under performance efficiency quality attribute, these usually refer to computational resources (e.g. CPU, storage, and network usage) which can be ambiguous if energy is perceived as a ``resource'' because it is a trade-off to the computational resources. 
%\keila{This new restructuring only has 2 less sub-subsections that the previous challenges list description version in sections/challenges.tex}
Explainability has emerged as quality attribute associated to machine learning and other AI-based systems. This attribute appears often associated with the quality of data used by such systems because of its runtime behavior dependency in~\cite{9609199}. In this work we adopt this quality attribute having this emergent definition in mind.


%https://ieeexplore-ieee-org.galanga.hvl.no/abstract/document/7936138

%https://www.sciencedirect.com/science/article/pii/S0164121217303072?casa_token=fpGb_2J3_TAAAAAA:dkRKo4HTTIVtBRFe9I2ly5dXGfMS-QZwhAwnJ0xV0nH9qg9vnJG-OY0LqUmI6_kTzspNEfCcrQ

%https://www.academia.edu/download/75105464/A_Software_Engineering_View_of_Data_Qual20211124-20629-1ykybxu.pdf

%https://www.sciencedirect.com/science/article/pii/S1474034622002592?via%3Dihub

%https://ceur-ws.org/Vol-1416/Session1Paper3.pdf

==> sections/challenges.tex <==
\section{Challenges}
\label{sec:challenges}
%\del{In this section, we introduce software and data product quality attributes from standardized quality models. Since these standardized models are not able to capture all the impacting concerns from the identified challenges, additional quality attributes from the literature are adopted for the purpose. Those are described in section~\ref{sec:QA}.
%Lastly, we describe main quality attributes negatively impacted by the identified challenges, describing their effect on the resulting software architecture. Table~\ref{tab:challenges} summarizes a total of fifteen challenges that were identified and analysed in terms of its impact to software and data quality attributes following the ISO/IEC standards. For the latter, the attributes are spread across three categories: inherent data quality (accuracy, completeness, consistency, currentness, and credibility), inherent and system-dependent data quality (accessibility, efficiency, compliance, confidentiality, precision, traceability, and understandability), and system-dependent data quality (availability, portability, and recoverability).}
%%Because of the intersectionality among the last two data quality dimensions quality attributes and the software ones, we have aggregated and discussed them by the software quality attributes. %discuss from image in: https://link.springer.com/article/10.1007/s11219-019-09494-x/figures/2
%\del{We have aggregated and discussed the impact on software quality attributes in conjunction with the last two data quality categories because of the perceived intersectionality among them. We complete the section with the discussion of impacted data inherent quality attributes in section~\ref{sec:intrinsics_QA}.}

%\subsection{\del{Quality Attributes}}
%\label{sec:QA}

The system behavior is highly dependent on data quality, and our aim is to analyse an architecture from the point of view of its heterogeneous data flows. We have therefore analyzed the gathered challenges using the quality attributes for software and data products from the ISO/IEC 25010~\cite{iso25010} and the ISO/IEC 25012~\cite{iso25012_2} quality models, respectively. We introduced two additional quality attributes on the quality model in order to accommodate challenges not captured by ISO/IEC 25010  and ISO/IEC 25012: Energy efficiency as suggested in~\cite{bass2003software} and Explainability from~\cite{9609199,habibullah2023non}. 

%While the sustainability of architectural decisions remain an open challenge and relates to the evolution of systems~\cite{VENTERS2018174}
%\rogardt{Why do we have this sentence above? It seems to come out of the blue. Next sentence is about energy efficiency and relate to previous paragraph. So that make sense. }\thanh{agree. I did not read the ref yet, but if it is about how data quality attributes affect the sustainability of software systems or software architecture, then it is fine. It is because we want to say that although the dimensions we picked are important but they are still missing and we introduce two more.}
The energy efficiency quality attribute is identified across different studies~\cite{bass2003software,VENTERS2018174,koccak2015integrating} as a characteristic to be considered when evaluating  of software systems as it contributes to the software sustainability. 
%\rogardt{How the last part is related to energy efficiency is not really clear.}\thanh{It is fine for me.} 
Although the ISO/IEC 25010~\cite{iso25010} encompasses a resource utilization sub-characteristic under performance efficiency quality attributes, but these usually refer to computational resources (e.g. CPU, storage, and network usage), which can be ambiguous if energy is perceived as a resource because it is a trade-off to the computational resources. 
Explainability has emerged as a quality attribute associated with machine learning and other AI-based components due to their ``black box'' characteristics. It is often associated with the quality of data used by such systems since its runtime behavior depends on data~\cite{9609199}, which influences the decision-making process of these systems. %In this work we adopt this quality attribute having this definition in mind. \lars{I think the last sentence can be omitted}

Next, we discuss 16 of the identified challenges in the lens of the software and the data quality attributes. % (highlighted in bold). 
The challenges and their impacted software and data quality attributes of \texttt{System} are summarized in Table~\ref{tab:challenges}. % and are referred throughout this section by their \texttt{ID} in bold.

\begin{table*}[h]
\caption{Software architecture relevant challenges on stationary wireless marine observing systems}
\label{tab:challenges}
\centering
\scriptsize
{
\centering
\begin{tabular}{|c|l|c|l|ll|l|}
\hline
\multirow{2}{*}{\textbf{ID}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Challenge}}} & \multirow{2}{*}{\textbf{Layer}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Quality of Software \\ Product Impacted\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Quality of Data Product Impacted}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{References}}} \\ \cline{5-6}
 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{Inherent}} & \multicolumn{1}{c|}{\textbf{System-dependent/Both}} & \multicolumn{1}{c|}{} \\ \hline
CH1 & Limited battery & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Underwater \\ Data Acquisition\end{tabular}} & Reliability (availability)& \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Accuracy,\\ Credibility,\\Completeness\end{tabular}} & Recoverability & \cite{ref2,ref3,ref5,ref11,ref13,ref14} \\ \cline{1-2} \cline{4-7} 
CH2 & Physical vulnerability &  & Reliability (availability) & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Accuracy,\\ Credibility,\\Completeness\end{tabular}} & Recoverability & \cite{ref3,ref4,ref5,ref7,ref8,ref11,ref14} \\ \cline{1-2} \cline{4-7} 
CH3 & Lack of device output format standards &  & \begin{tabular}[c]{@{}l@{}} Compatibility \\ (Interoperability)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness,\\Consistency\end{tabular}}  & \begin{tabular}[c]{@{}l@{}} Compliance \\ Portability\end{tabular} & \begin{tabular}[c]{@{}l@{}} \cite{ref3,ref5,ref7} \\ \cite{ref14,ref15} \end{tabular} \\ \hline % \cline{1-2} \cline{4-7} 
%\multicolumn{1}{|l|}{CH3} & IoUT equipment environmental impact &  & \begin{tabular}[c]{@{}l@{}}Performance efficiency \\ (resource utilization)\end{tabular} & \multicolumn{1}{l|}{Credibility} & Compliance &  \\ \hline
CH4 & Unreliable UAC links &  & \begin{tabular}[c]{@{}l@{}} Reliability (Fault \\Tolerance) \end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\Completeness\end{tabular}} & Recoverability & \begin{tabular}[c]{@{}l@{}} \cite{ref2,ref4,ref5,ref7} \\ \cite{ref9,ref10,ref11,ref14} \end{tabular} \\ \cline{1-2} \cline{4-7} 
CH5 & Missing raw data & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Network \\ Communication\end{tabular}}  & Explainability* & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness\end{tabular}} & Understandability  & \cite{ref13,ref14} \\ \cline{1-2} \cline{4-7} 
CH6 & Environmental impact of UAC & & \begin{tabular}[c]{@{}l@{}}Performance efficiency \\ (resource utilization)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\Completeness\end{tabular}} & N/A & \cite{ref1,ref5,ref14} \\ \cline{1-2} \cline{4-7} 
CH7 & \begin{tabular}[c]{@{}l@{}}Low communication bandwidth and \\ high latency of UAC and OTA links\end{tabular} &  & \begin{tabular}[c]{@{}l@{}}Performance efficiency \\ (capacity)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility, \\ Currentness\end{tabular}} & N/A & \cite{ref6,ref13,ref14,ref16} \\ \cline{1-2} \cline{4-7} 
CH8 & Security vulnerability of UAC links &  & Security & \multicolumn{1}{l|}{Credibility} & \begin{tabular}[c]{@{}l@{}}Availability, \\ Confidentiality\end{tabular} & \begin{tabular}[c]{@{}l@{}} \cite{ref3,ref6,ref11,ref12} \\ \cite{ref14,ref19} \end{tabular} \\ \cline{1-2} \cline{4-7} 
CH9 & Power-hungry UAC data transmission &  & Energy efficiency* & \multicolumn{1}{l|}{Credibility} & Recoverability & \cite{ref3,ref10,ref14} \\ \hline
CH10 & Complex data usage & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Data \\ Management\end{tabular}} & \begin{tabular}[c]{@{}l@{}} Usability (Appropriateness \\ recognizability)\end{tabular} & \multicolumn{1}{l|}{N/A} & Understandability & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
CH11 & Lack of automatic QC procedures &  & N/A & \multicolumn{1}{c|}{\textbf{All}} & \multicolumn{1}{c|}{\textbf{All}} & \cite{ref13,ref14,ref15,ref17} \\ \cline{1-2} \cline{4-7} 
CH12 & Heterogeneous data sources & &  \begin{tabular}[c]{@{}l@{}} Compatibility \\ (Interoperability)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Credibility,\\ Completeness,\\Consistency\end{tabular}} & \begin{tabular}[c]{@{}l@{}} Compliance \\ Portability\end{tabular} & \cite{ref13,ref15,ref18} \\ \cline{1-2} \cline{4-7} 
CH13 & \begin{tabular}[c]{@{}l@{}}Sensitive data \\ (Business and Defense critical)\end{tabular} &  & Security & \multicolumn{1}{l|}{N/A} & \begin{tabular}[c]{@{}l@{}}Availability, \\ Confidentiality\end{tabular} & \cite{ref13,ref15} \\ \cline{1-2} \cline{4-7} 
%CH15 & \begin{tabular}[c]{@{}l@{}}Lack of marketplace for \\ data sharing and selling\end{tabular} &  & Usability (accessibility - of data) & \multicolumn{1}{l|}{N/A} & Accessibility & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7}
CH14 & Data reusability &  & Reusability & \multicolumn{1}{l|}{N/A} & \begin{tabular}[c]{@{}l@{}}Availability, \\ Confidentiality\end{tabular} & \cite{ref13,ref14,ref15} \\ \cline{1-2} \cline{4-7} 
CH15 & Access control for data sharing &  & Security & \multicolumn{1}{l|}{N/A} & \begin{tabular}[c]{@{}l@{}}Availability, \\ Confidentiality\end{tabular} & \cite{ref13,ref15} \\ \hline
\end{tabular}
}
\begin{tablenotes}
      \item \scriptsize
*  -- New adopted QA \(|\)  Abbreviations: UAC (Underwater Acoustic Communication); OTA (Over-The-Air); N/A (Not Applicable).
\end{tablenotes}
%\vspace{-0.5cm}
\end{table*}

% \subsection{Software Product and Data Product System-dependent Quality Attributes Impacted}
% \label{sec:system_QA}
%\keila{Merging both attributes because of their intersectionality}

%\paragraph{Compatibility}
\subsection{Compatibility}
\label{sec:compatibility}
\textbf{Compatibility} of \texttt{System} %concerns interacting components in the system and affects the interoperability in two different layers. Firstly, it 
is affected in the underwater data acquisition layer because of the sensor integration. It implies that heterogeneous communication protocols and associated output data formats need to be unified at the UWSN level to ensure a common syntax and semantics within data producers' sub-systems (\textbf{CH3}). %Secondly, i
It affects also the data management layer as the originating dataset from the integration of measurements from different sensors is supplied by data producers' sub-systems in various formats. %fields differing in their meaning semantics. 
Additionally, there might be different types of data, such as time series, images, or videos, which are categorized into point-based and array-based data~\cite{ref15}. At the cloud service level, where multiple data sources are merged, interoperability is required to ensure that the different processing components interpret data based on the same metrics and criteria (\textbf{CH12}).
When data has proprietary or organization-dependent syntax and semantics, its \textbf{compliance} to standards and \textbf{portability}, i.e., ``\textit{degree to which data has attributes that enable it to be installed, replaced or moved from one system to another}''~\cite{iso25012}, can be affected.

%\paragraph{Explainability and Usability}
\subsection{Explainability and Usability}
\label{sec:explainability}
Because of the low %underwater communication 
bandwidth and high propagation delay of UAC at the UWSN level, 
%\rogardt{Neither local processing and aggregation need to reduce the data amount? Is is not the case that not all data is sent that is the main reason, such as, for example, just send up an alarm is something is happening? Or just identify from a picture how many fish there are and send up the number of fish? }
%there is often local processing and aggregation of data to reduce the data volume such that only important information or events are sent up the data delivery chain.
there is an aggregation or local processing of data to filter important information or events, which will be sent up the data delivery chain. The raw data is often kept for retransmission and can be retrieved during recovery or maintenance of the sensing platforms at sea. Despite that, storage might also be an issue when operating over a long time. Since the raw data records can be crucial for data analytics tasks, their absence can have implications in the \textbf{understandability} of data and the \textbf{explainability} of automatically detected phenomena or actions performed based on the data (\textbf{CH5}). 
Lack of metadata, which can provide information regarding the required data quality inherent dimensions hindering its adequate use for a specific context, is another challenge affecting \textbf{understandability} (\textbf{CH10}).
%Another challenge affecting the \textbf{understandability} of data is complex data usage derived from the lack of metadata that can provide information regarding the required data quality inherent dimensions hindering its adequate use for a specific context (\textbf{CH10}).\lars{I do not understand the last sentence} 
These challenges impact the \textbf{usability}, and more specifically the ability to ``\textit{recognize whether a product or system is appropriate for their needs}''~\cite{iso25010}. 
Also, a lack of explainability of current procedures makes it difficult to fully automate data quality control procedures (\textbf{CH11}).
%On the other hand, the lack of data quality control (\textbf{CH11}) procedures is impacted by the lack of explainability of current procedures, making it difficult to fully automate them. 
Because of the high complexity of data, such activities currently require domain experts' intervention and usually cause delays of up to six months. This makes the process subjective and strongly dependent on the experience of the person in charge. 
%In addition, the practitioners admitted that performing data quality control is subjective and mostly based on the perspectives and experiences of the person in charge. 
Since marine data is prone to errors due to the uncertainty of the environment and to % various environmental impacts and 
technological constraints, existing procedures often focus on assessing the inherent characteristics of data.  
%Besides, existing communication technologies are unreliable and may generate noise during data transmission. 
Still, it is of high importance to perform data quality control before employing the data further considering the quality dimensions required for its context of use.
%\lars{what does not means when we hae a sentence like this in bold?}

%\paragraph{Reliability and Performance efficiency}
%\subsection{Reliability and Performance Efficiency}
\subsection{Recoverability}
\label{sec:reliability}
\textbf{Recoverability} data quality attribute, i.e., ``\textit{the degree to which data has attributes that enable it to maintain and preserve a specified level of operations and quality, even in the event of failure}''~\cite{iso25012}, is impacted by challenges affecting  \textbf{reliability}, \textbf{performance efficiency}, and \textbf{energy efficiency} software quality attributes.
Firstly, regarding \textbf{performance efficiency} (\textbf{resource utilization}), the noise generated by the communication device's signals can negatively impact species that use acoustics to communicate or prey, e.g., by leading them to confusion or causing other changes in the behavior (\textbf{CH6}). Because of the impact of the underwater acoustic signals on marine life, there could be restrictions on the transmission windows and frequencies. This challenge has implications on the communication channels and links utilization.

Furthermore, in the network communication layer, wireless communication channels in IoUT have less available bandwidth per packet transmission (\textbf{CH7}) compared to traditional land-based channels. This is the case for the acoustics in underwater communications and satellite in over-the-air communication (OTA), where latency can vary according to atmospheric or water conditions (e.g. affected by absorption). Lastly, the OTA options (satellite and mobile networks) to transmit data into IP networks usually have higher costs associated with the carrier service. These challenges constrain the overall network \textbf{performance efficiency capacity} of software systems in IoUT environments.

When it comes to \textbf{reliability} at the underwater data acquisition layer, the only power source for underwater equipment is the battery. This limited resource lifetime can vary from a few weeks to years depending on the data sampling rate, the precision of instruments, and the power consumption of the transmission device (\textbf{CH9}). This last factor is due to the higher consumption of energy associated with transmission devices when compared to computation done locally. Thus, \textbf{energy efficiency} is one of the main drivers of the overall system.
%\thanh{hard for me to link limited energy to reliability, isn't it still about performance efficiency?}
%This challenge forces software embedded in sensor nodes to optimize power consumption, which includes managing processing and transmission tasks. Regarding these tasks, there are indications that transmission devices consume more energy than computation, and components can be temporarily powered off to save energy (sleep mode)~\cite{ref14}.
Additionally, at the UWSN level, underwater sensors, communication modems, and gateways are vulnerable to physical impacts. For example, equipments can be damaged by human activities (e.g., hit by ships) or by nature (e.g., dragged by sea waves, currents, or ice). This can affect sensor measurements, device integrity and their resulting data quality. 
%\thanh{it becomes a bit clearer here for reliability, but I agree with Rogardt that there is no link between reliability and performance effienciency.}
%\thanh{the discussion seems to back and forth. First, it was about performance efficiency, then reliabity, and now performance efficiency again. Would that be possible to link them here? The next paragraph seems to better do the job.} 

In summary, while the physical vulnerability (\textbf{CH2}) of the hardware and the limited battery (\textbf{CH1}) affects the availability of the software system (its operation), the unreliability associated with the wireless underwater network links (\textbf{CH4}) impacts the capacity of the software system to operate in the presence of faults in the communication channel. %recoverability implication as well 
%\rogardt{What do recoverability have to do with Reliability and Performance Efficiency?}

%Moreover, the power-demanding UAC transmissions (\textbf{CH9}) is a failure which could impact data availability.  %\paragraph{Energy efficiency}
%Transmissions must be handled carefully to avoid the drainage of the battery power because communication devices can be the component that consumes more energy in the systems at the UWSN level. 
%As pointed out in~\cite{bass2003software}, \textbf{energy efficiency} of software systems can no longer be disregarded.
%In the marine domain, \textbf{energy efficiency} is one of the main drivers of the overall system because of its implication on the availability of the systems and the data produced by them due to the risk of power down and the time and costs to its maintenance.\lars{This last sentence appears a bit otu of context for me - it is a bit forth and back?} % (e.g. battery replacement operations). 
%\paragraph{Security}
\subsection{Security}
\label{sec:security}
When it comes to \textbf{security} at the network communication layer, UAC is susceptible to a range of attacks (\textbf{CH8}) including packet capture, routing attacks, and blockage of a link between nodes (DoS) due to the accessibility to the wireless channel. 
%Authentication should be done but the land-based network authentication methods implementation in this context is not trivial due to the communication overhead. Other detection and mitigation can be implemented to circumvent the openness of the communication channel, but these also increase the communication overhead underwater which is already restricted, specially in the case where there are many nodes in the network.
Authentication and detection strategies can be implemented to mitigate the open UAC communication channel and spoofing of sensor nodes. However, implementing land-based network security methods in this context is not trivial due to the communication overhead underwater, especially when there are many nodes in the network.
A detailed description of the types of attacks and their mitigation can be found in~\cite{ref19}.  At the data management layer, two interrelated challenges impact security in terms of confidentiality and rightful access to data being shared: (i) the access to data being collected needs to be carefully filtered in terms of its category (\textbf{CH15}), and (ii) 
%Because of the need to share data beyond the initial context it was acquired motivated by regulations, better forecast and safety measures on organizations' operations areas, or to adhere to initiatives to provide data for climate and marine sciences for better public perception (\textbf{CH14}).\lars{I cannot make sense of this last sentence}
data categorization and filtering are motivated by data sharing beyond the initial context in which it was acquired (\textbf{CH14}). Some reasons behind this are regulations, better forecast and safety measures on organizations' operations areas, or adhering to initiatives to provide data for climate and marine sciences for better public perception.
In summary, the data to be shared could be categorized into (\textbf{CH13}) legally restricted, business-critical, or open-access data. An example of legally restricted data is data that is critical for the maritime territory defence because it details the bathymetry of a specific region at the sea, or stock market data. Open-access data refers to ``non-footprint'' data valuable to a third-party entity or to new applications, which requires resources to be shared.
    % \begin{itemize}
    %     \item \textbf{Legally restricted} -- Data that cannot or has to be shared to compliance with laws and regulations. An example is data that is critical for the maritime territory defence of a country because it details the bathymetry of a specific region at sea.
    %     \item \textbf{Business critical} -- Data that contains critical information for business operations, e.g. ``sensitive data''. This type of data is critical not only for data owners but also for data producers to improve sensor measurements at the data acquision layer.
    %     \item \textbf{Open-access data} -- Data that can cause no harm to sharing entity, e.g. ''non-footprint'',  and can be valuable to a third party entity or to new applications, but requires resources to be shared. This data, of is not being sent can be easily overwritten since storage can also be a constraint in the sensing devices or at the gateways in the edge.
    % \end{itemize}
In terms of data-related quality attributes, these challenges impacts data \textbf{availability}, i.e. ``\textit{the degree to which data has attributes that ensure that it is only accessible and interpretable by authorized users}''~\cite{iso25012}; and \textbf{confidentiality}, which is defined as ``\textit{The degree to which data has attributes that enable it to be retrieved by authorized users and/or applications}''~\cite{iso25012}.

\subsection{Data Product Inherent Quality Attributes Impacted}
\label{sec:intrinsics_QA}
% \keila{use RE table}
\paragraph{Accuracy}
This quality attribute is impacted by all challenges that affect the sensor measurements, deviating the measurements from the observed phenomena aimed to be captured. For example, bio-fouling concerns microorganisms growing around underwater sensors. It is an unavoidable problem for artificial objects operating in the ocean. When a sensor experiences that issue, it will produce \textbf{inaccurate} measurements which can lead to errors such as data drift. Another example of factors impacting data accuracy is the sensor power supply. If a battery is running low and there are inconsistencies to the sensor energy supply, there might be errors introduced in the sensors' readings, which in turn originates erroneous data. Lastly, the physical vulnerability also affects the positioning of the sensors and thus can have a negative implication on the reading. For instance, sensors deployed close to the water surface may accidentally make a reading outside of the water. Another example concerns sensors that use their static configured position as part of the data acquisition and are dragged from their initially deployed location.

\paragraph{Completeness, Consistency and Currentness}
These quality attributes are impacted by all challenges affecting the reliability and performance (in terms of network throughput) quality attributes of the data-producing system. %at the data acquisition and network communication layers. 
The reason is that these challenges entangle the availability of software components and data transmission. The compatibility-related challenges can affect the \textbf{completeness} of the data products because of the lack of common fields and metadata available from the heterogeneous sources of data at the data acquisition and management layers. In addition to the compatibility challenges,  \textbf{consistency} with other data might be affected as well because of the correlation of measurements.
%Additionally, when the \textbf{completeness} is affected in this context, because of the correlation of measurements the \textbf{consistency} with other data might be affected as well. 
Finally, the high latency associated with the underwater and OTA communication channels greatly impacts the arrival time of data to data consumer applications. This in turn affects the \textbf{currentness} data quality attribute.

\paragraph{Credibility}
\textbf{Credibility} is a cross-cutting inherent data quality attribute, and it relates to ``\textit{truthfulness of origins}''~\cite{iso25012}. In the IoUT context, it is not possible to have ground truth for all measurements and most quality control procedures focus on investigating the closeness of the data to its true value~\cite{ref17}. % covering the inherent characteristics of data.
%Regarding trust, 
Trust is also %other studies have also 
%considered as 
impacting the cross-organizational level of the system because of all the uncertainty affecting the data streams until its (re)use~\cite{ref13}.
%In contrast other studies consider credibility as an attribute related to systems' trust and thus recommend that it must be perceived as an external quality attribute (system-dependent).
%This topic needs to be further investigated as it remains an open-challenge and goes beyond the scope of this paper.\lars{should this last sentence be here or possibly in future work?} %in the software and data quality research, 



==> sections/decisions.tex <==
\section{Architectural Decisions}
\label{sec:decisions}
 %We now provide a detailed description of the rationale behind the architectural decisions that resulted from the process described in Section~\ref{sec:method}. 
 
 In this section, we describe the main architectural decisions to build systems exploiting heterogeneous marine data streams. The decisions are summarized in Table~\ref{tab:decisiosn}. All decisions are made by considering the challenges presented in the previous section and thus aid in mitigating the system's quality attributes affected. The architectural decisions do not address the challenges in isolation but, instead, in context with other conflicting or related challenges. %They also consider stakeholders’ needs and feedback, being incorporated into the architecture for integration with existing components and legacy systems. %\lars{This last sentence is very long and it is hard to understand the last part}
% In Figure~\ref{fig:legend}, we present the legend for the architecture overviews provided throughout the paper. We combined the component-and-connector view with an allocation and organizational flow view.
 Throughout the description of architectural decisions, we also refer to a component and connector view shown in  Figure~\ref{fig:arch}, which highlights the data flow components.
 
 
% highlight their connection with the component-and-connector and organizational flow view shown in % explain how these appear in the resulting architecture layout as shown in the overview in 
% Figure~\ref{fig:arch}. 
  
%Furthermore, architectural decisions describe the rationale, risks, and assumptions made during the design process of a software system. This description is crucial not only for the implementation stage but also for the analysis of the architecture, especially in its maintenance~\cite{bass2003software}. %trade-offs as well

\begin{table}[hb!]
\caption{Summary of Architectural Decisions (ADs)}
\label{tab:decisiosn}
\centering
\footnotesize
{
\centering
\begin{tabular}{|p{.5cm}|p{5cm}|p{2cm}|}
\hline
\textbf{ID} & \textbf{Architectural Decision} & \textbf{Challenges}\\ \hline
AD1 & Distributed data processing and transmission responsibilities & {\scriptsize CH1,CH4,CH5,CH6, CH7,CH8,CH9}  \\ \hline
AD2 & Data platform & {\scriptsize CH12} \\ \hline
AD3 & Message-oriented data ingestion middleware & {\scriptsize CH1,CH2,CH9} \\ \hline
AD4 & MQTT messaging protocol & {\scriptsize CH4,CH7,CH9}  \\ \hline
AD5 & Platform monitoring & {\scriptsize CH1,CH2,CH4, CH12,CH13,CH15}  \\ \hline
AD6 & Data quality control & {\scriptsize CH5,CH11,CH12} \\ \hline
AD7 & Data model for integrated data sources & {\scriptsize CH3,CH10,CH12} \\ \hline
AD8 & Identity provider & {\scriptsize CH13,CH15}  \\ \hline
AD9 & Data sharing access control & {\scriptsize CH13,CH14,CH15}\\ \hline
AD10 & Data classification and triage & {\scriptsize CH13,CH14}  \\ \hline
\end{tabular}
}
\end{table}

%\keila{Add column impact: cross-organizational or inter-organizational (i.e., data provider, data producer, service/platform provider)}
%\begin{table}[hb!]
%\caption{Summary of Architectural Decisions (ADs)}
%\label{tab:decisiosn}
%\centering
%\scriptsize
%{
%\centering
%\begin{tabular}{|l|l|l|l|}
%\hline
%\multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Architectural Decision}} & \multicolumn{1}{c|}{\textbf{Challenges}} \\ \hline
%AD1 & \begin{tabular}[c]{@{}l@{}}Distributed data processing and transmission\\  responsibilities\end{tabular} & \begin{tabular}[c]{@{}l@{}}CH1, CH4, CH5, CH6, \\ CH7, CH8 CH9\end{tabular}  \\ \hline
%AD2 & Data platform & CH12 \\ \hline
%AD3 & \begin{tabular}[c]{@{}l@{}}Message-oriented data ingestion middleware\end{tabular} & \begin{tabular}[c]{@{}l@{}}CH1, CH2, CH9\end{tabular}  \\ \hline
%AD4 & MQTT messaging protocol & \begin{tabular}[c]{@{}l@{}}CH4, CH7, CH9\end{tabular}  \\ \hline
%AD5 & Platform monitoring & \begin{tabular}[c]{@{}l@{}}CH1, CH2, CH4, CH12,\\CH13, CH15\end{tabular}  \\ \hline
%AD6 & Data quality control & \begin{tabular}[c]{@{}l@{}}CH5, CH11, CH12\end{tabular}  \\ \hline
%AD7 & Data model for integrated data sources & \begin{tabular}[c]{@{}l@{}}CH3, CH10, CH12\end{tabular}  \\ \hline
%AD8 & Identity provider & CH13, CH15  \\ \hline
%AD9 & Data sharing access control & CH13, CH14 CH15\\ \hline
%AD10 & Data classification and triage & CH13, CH14  \\ \hline
%\end{tabular}
%}
%\end{table}

% \begin{figure}[htb!]
%     \centering
%     % [trim={left bottom right top},clip]
%     \includegraphics[trim={5cm 1.2cm 0cm 10.2cm},clip,width=\linewidth]{figures/notation.pdf}
%     \caption{Component-and-connector structure notation.}
%     %\pat{where do we refer this figure and what is it?} %data actor role and allocation view
%     \label{fig:legend}
% \end{figure}

\begin{figure*}[htb!]
    \centering
    % [trim={left bottom right top},clip]
    \includegraphics[trim={0cm 0.25cm 0.5cm 0.25cm},clip,width=0.8\linewidth]{figures/arch_overview.pdf}
    \caption{Overview of the resulting architecture (component and connector view).} %Component-and-connector 
    \label{fig:arch}
\end{figure*}

\paragraph{Distributed data processing and transmission (AD1)}
%\lars{AD1 description is very long. Perhaps we should try to make each AD description approx. the same lenght}
%Assumption: data is considered the measurement value (after signal conversion - output of sensor)
%When migrating, building, or deploying a system for real-time in situ marine data acquisition and sharing in a cross-organizational context, 
%These constrains boils down to a optimization problem between the amount of data to be sent, the transmission rate
%influences the sampling rate?
%also addressing the quality attributes affected by the specificity introduced by the challenges at the first two layer of the overall system:
% \begin{itemize}
%     \item Volume, resolution, and throughput of data
%     \item Environmental impact of communication + number of devices
% \end{itemize}
%Depends on the configuration, deployed capability, and operational scenario requirements:
%Should have the possibility to send only "data diffs" (changes in data) -  tradeoff between energy efficiency, data availability and volume (compression) - reconstruct information if needed* - reduce impact on the environment
%One should consider the following concerns regarding the configuration of the software components involved in the data acquisition and the data delivery chain to meet the operational scenarios. These components can help address the challenges associated with data acquisition and network communication, which constraints impose tradeoffs on the resulting software architecture. 
%There are many concerns to be balanced when implementing the components in the data acquisition and network communication layers, in order to meet the operational scenarios requirements.
Because of the challenges at the data acquisition and network communication layers, there is a tradeoff to be done among the volume of data sent, the power consumption to transmit data (\textbf{CH9}) in the UWSN, and the density of the wireless communicating nodes in the area to cover and their impacts when transmitting data wirelessly (\textbf{CH6}). On the one hand, the volume of data depends on the number of sensor devices deployed, their configured sampling rate, security mitigation strategies (\textbf{CH8}), and the power consumption in the nodes inside the UWSN (\textbf{CH1}). These aspects are part of the responsibilities of the  \textsf{\small Sensor} component in the overall architecture layout in Figure~\ref{fig:arch}.
%On the other hand, the available bandwidth and latency can vary with the water's physical properties being in best conditions already very limited when compared to the amount of data that can be generated or the bandwidth available in typical land-based systems, creating a bottleneck in the throughput (\textbf{CH4} and \textbf{CH7}). Lastly, each transmitted message inside the UWSN can impact the life and the surrounding ecosystem. This decision brings computation closer to data acquisition instead of sending raw data to be processed on the cloud level where more resources are available (\textbf{CH5}). The  \textsf{\small Local Processing} component in the  architecture depicted in Figure~\ref{fig:arch} is a consequence of this, being responsible for aggregating and fusing raw measurement data from the different sensors in UWSN. Local computation is associated with the transmission of data because of the limited wireless communication options and the unfeasibility and cost of employing wired communications from sea to shore. 
On the other hand, the available bandwidth and latency can vary with the water’s physical properties being in best conditions already very limited when compared to the amount of data that can be generated or the bandwidth available in typical land-based systems, creating a bottleneck in the throughput (\textbf{CH7}). Additionally, each transmitted message inside the UWSN can impact marine life. 
The  \textsf{\small Local Processing} component in the architecture depicted in Figure~\ref{fig:arch} is a consequence of this, being responsible for aggregating and fusing raw measurement data from the different sensors in the UWSN. Because of the limitations on data transmission (\textbf{CH4} and \textbf{CH7}), this decision brings computation closer to data acquisition instead of sending raw data to be processed on the cloud level where more resources are available (\textbf{CH5}).
%When it comes to the transport inside the UWSN, \textit{ad hoc} protocols are needed when transmitting data from underwater to surface gateways. There is also a need to serialize the data for the different communication channels and devices. This behavior is part of the responsibilities of the  \textsf{\small Communication Management} component depicted in Figure~\ref{fig:arch}, which is also responsible for bridging data between different physical channels, e.g., underwater acoustics and over-the-air technologies. In turn, the surface gateways have to bridge to long-range transmission channels provided by satellite links or mobile networks (e.g. 4G or 5G) using the carriers' standardized APIs.
When it comes to the transport inside the UWSN, \textit{ad hoc}  protocols and serialization are needed when transmitting data from underwater to surface gateways. In turn, the surface gateways have to bridge to long-range transmission channels provided by satellite links or mobile networks (e.g., 4G or 5G) using the carriers' standardized APIs. This behavior is part of the responsibilities of the  \textsf{\small Communication Management} component depicted in Figure~\ref{fig:arch}, which is responsible for bridging data through heterogeneous communication channels and devices, e.g., underwater acoustics and over-the-air technologies. 


\paragraph{Data Platform (AD2)} To address the interoperability issue introduced by challenge \textbf{CH12}, there was a decision to have a data platform built to allow data aggregation from different sources before its usage on the application level in the different use cases within the marine domain. The rationale behind this decision was to have a common configurable platform that can be parametrized when interfacing with the other layers according to its operational scenario requirements. Although some processing is done in the lowest layers, at the platform level, data fusion is performed, aggregating data from different sensing platforms. Thus, it is assumed that the volume of data is greater at this level despite sharing the property of dealing with heterogeneous data formats at device and data source ingestion, accordingly. In the resulting architecture presented in Figure~\ref{fig:arch}, this decision is reflected in the  \textsf{\small Ingested Data Processing}, and the  \textsf{\small Data Space} on the right side.
%
\paragraph{Message-oriented data ingestion middleware (AD3):} 
The rationale for this decision was to use a standardized way to provide data that is delivered by different (distributed) systems to  \textsf{\small Data Consumer Application}s. By using the publish-subscribe pattern, we decouple data-producing systems from data-consumer systems, bringing more flexibility when handling outages from each one of these types of systems. With this pattern, data producers and consumers do not need to know or keep information about each other, transferring the responsibilities to a broker component that can also handle concurrent data ingestion and provisions to the different systems that might connect to it over time. The resulting architecture presented in Figure~\ref{fig:arch} implements this component via the  \textsf{\small Ingestion Broker}. This decision adapts to the uncertainty introduced by unreliable communications and the physical vulnerability of the components in the underwater data acquisition and the network communication layers (\textbf{CH1}, \textbf{CH2}, and \textbf{CH9}), affecting data reliability and availability.
%\del{, on the software and system-dependent data quality side respectively}\eric{or split into several sentences}.
%
\paragraph{MQTT Protocol (AD4)} MQTT is an OASIS standard protocol for message exchange in IoT-enabled systems and it is used on the top of the publish-subscribe communication model pattern. Its lightweight (low footprint and small message size) characteristics and simplicity in implementation have fomented the creation of a large community and services built on top of the protocol~\cite{mqtt_survey}. Other important characteristics of the protocol are the Quality-of-Service (QoS) levels for end-to-end communication: 
%\footnote{The QoS levels are applied to the sender and receiver of the message (publisher-broker or broker-subscriber), and thus the end-to-end quality of service level must be implemented on the top of the protocol usage.\eric{footnote does not add much for me. Elaborate or remove?}}: 
Level 0 (at most once) is suitable for operational scenarios in which data loss is permitted; Level 1 (at least once) can be used in operational scenarios in which duplicated data delivery is permitted; and Level 2 (exactly once) in cases in which data duplication is not suitable.
% \begin{itemize}
%     \item At most once (level 0) -- should be used in operational scenarios that data loss is permitted.
%     \item At least once (level 1) -- should be used in operational scenarios that duplicated data delivery is permitted.
%     \item Exactly once (level 2) -- should be used in operational scenarios that requires assure of data delivery without duplicates.
% \end{itemize} 
Depending on the network protocol inside the UWSN that defines the behaviour for re-transmissions for the surface gateway systems, it might be more adequate to deploy the different QoS levels from the communication between the  \textsf{\small Surface Gateway} and the  \textsf{\small Ingestion Broker} component, and addressing the uncertainty introduced by the unreliable underwater wireless communication (\textbf{CH4}).
The low footprint also fits well with the low communication bandwidth and high operation costs of the satellite link (\textbf{CH7}), and contributes to its low overhead to save bandwidth and potentially the number of transmissions needed (\textbf{CH9}).
%These characteristics were behind the selection of the protocol for the transmission of data from the different data producers' devices at sea, and into the data platform. Furthermore, t
The size of the data to be transmitted also influences %is also taken %was also took 
%into consideration for 
the selection of a suitable network protocol solution.

\paragraph{Platform monitoring (AD5)}
The main drivers for this decision are the different causes of faults that impact the layers inside the UWSN, affecting the availability of data on the  \textsf{\small Ingested Data Processing} component. Since there is a runtime dependency of the system behavior on data, it is crucial to detect errors that occur in runtime as early as possible to trigger context information for root cause analysis and shorten the recoverability of the overall system. More specifically, it addresses the challenges at the data acquisition and network layers,  causing uncertainty in the data availability introduced by unreliable communication, physical vulnerability, and limited battery (\textbf{CH1}, \textbf{CH2}, and \textbf{CH4}).
This decision also encompasses the monitoring of the interactions of the data platform with the external systems. Not only the ingestion of data (\textbf{CH12}) but also the consumption of data to help access the usage of the overall data management layers components to provide data to the rightful consumer applications systems (\textbf{CH13} and \textbf{CH15}). For this decision to be implemented, components and data instrumentation, i.e., measurement and recording of their runtime outputted behavior, are needed. Thus, intervention in the different parts of the architecture is required, becoming a cross-cutting concern.

\paragraph{Data Quality Control (AD6)}
Data quality is one of the main drivers and concerns of stakeholders across various organizations. It is reflected in challenge \textbf{CH11}, and understanding it for the various marine use cases is crucial for trusting the decisions made on the provided data. In this domain, because of the restricted wireless underwater communication, there is an additional level of complexity when trying to understand the data quality because of the small volume of data that can be ingested into the data management layer (\textbf{CH5}). Knowledge about the UWSN must be kept and updated to be used during the quality control process, and this task can be distributed across the
different processing components ( \textsf{\small Local Processing} and  \textsf{\small Stream Processing}) layout in the overall architecture depicted in Figure~\ref{fig:arch}.  In particular, metadata information about the measurement systems (sensors) is needed to understand the level of data quality and its suitability for a specific use case. Additional contextual metadata information recorded throughout the data delivery pipeline ( \textsf{\small Monitoring}) and other related historical data sources might be used to assess and ensure the quality of the data on the real-time data streams. Furthermore, the different data source format standards (\textbf{CH12}) also affect the understanding of data adequacy according to the available information contained in the format for its use in the context of the different use cases.

%This decision reflects in the  \textsf{\small Stream Processing} component at the data management layer in the overall architecture layout in Figure~\ref{fig:arch}.
\paragraph{Data model for integrated data sources (AD7)}   
 On one hand, as a result of the  \textsf{\small Local Processing}, there is a resulting data source in a proprietary format for each organization that is then integrated for the different  \textsf{\small Data Consumer Application}s. The integration is needed because data producers have to incorporate sensors manufactured by others and deal with different device output formats (\textbf{CH3}). On the other hand, as a consequence of the diverse data formats and standards used to ingest data from the UWSN (challenge CH12), there was a need to have a uniform format for the processing done by the different services inside the  \textsf{\small Stream Processing}. This simplifies the development of the services upon a single format, and addresses and fosters a single understanding of the data at the data management layer. This decision aims to create a representative and flexible model to provide an adequate level of understanding (metadata) of data and its quality, addressing the challenges of the understandability of data for the different use cases (\textbf{CH10}). However, a challenge introduced by this decision is handling the model evolution as required information and available fields change over time and keeping backward compatibility to expected formats on the  \textsf{\small Data Consumer Application} side. Another consequence of this decision was the separation of the brokers, isolating  \textsf{\small Ingestion Broker} from  \textsf{\small Core Broker}. 

\paragraph{Identity provider (AD8)}
For the ingestion and sharing of the data in the data platform, there must be mechanisms to verify the identity of the systems interacting. There is also a need to ensure correct access, which can only be managed by knowing the identity of the systems. As the data platform and intermediary component with knowledge about data producers and  \textsf{\small Data Consumer Application}s, it can be used in the management of access to the data streams, addressing the access control challenge (\textbf{CH15}) on the one hand and establishing a baseline for the selective process of sharing sensitive (\textbf{CH13}) or insensitive data.
During the integration of the systems in various organizations, there was also an interoperability issue among the different authentication methods and solutions. The rationale behind this decision was to unify the authentication of components and their associated authorization to the different ingested and data sharing flows. Additionally, since various frameworks can be deployed between the decoupled high-level components in the architecture presented in Figure~\ref{fig:arch}, especially for the ones at the cloud level, the authentication solutions provided by those must also be integrated.
Therefore, this is a cross-cutting concern for the interactions between the components.


\paragraph{Data sharing access control (AD9)}
When data is delivered to the  \textsf{\small Data Consumer Application} component, there is a need for mechanisms to authorize access to the different flows of data (\textbf{CH15}) according to the data category and its degree of ``openness''. This decision helps to address challenges in accessing or vetting sensitive
data (\textbf{CH13}) and managing the ingestion into the  \textsf{\small Data Consumer Application}'s side because of the reusability challenge (\textbf{CH14}). This decision depends on an identity solution for the interacting systems and thus is closely related to the previous one (AD8), and together, they constitute a cross-cutting concern regarding ensuring security at the data management layer. 
%Because of the reusability introduced by challenge CH15, not all data can simply be forward to the  \textsf{\small Data Consumer Application}, and thus
%This decision’s behavior is implemented via the  \textsf{\small Identity Provider and Access Control Management} component presented in the architecture overview in Figure~\ref{fig:arch}.
Being the  \textsf{\small Identity Provider and Access Control Management} a cross-cutting concern presented in the architecture overview in Figure~\ref{fig:arch}, its implementation is done by adding authentication on the different components and sub-components, and by adding authorization to data accordingly. This decision encompasses rules defined at the authentication and authorization management, integrating with the various ways to deliver data via the  \textsf{\small Core Broker} and the  \textsf{\small Data Space} using the push and pull methods to the  \textsf{\small Data Consumer Application}. Moreover, this might also imply granularity of controls at brokers' topics access.

\paragraph{Data classification and triage (AD10)}
Complementary to the access control decision (AD9), an intermediary step is needed to classify the ingested data streams. One of the major drivers behind this decision is the sensitive data (\textbf{CH13}) because of its reusability (\textbf{CH14}) in a context different from the one for which the data acquisition was designed. The rationale for this decision is to filter different categories, quality levels, and ``openness'' of data impacting the access control to data shared on the  \textsf{\small Data Consumer Application} components. In the resulting architecture in Figure~\ref{fig:arch}, the  \textsf{\small Stream Processing} component is responsible for implementing the behavior behind the rationale of this decision.









==> sections/discussion.tex <==
%\subsection{Quality Attributes} -- discussion
%Gaps exist in particular for addressing data quality and its design consequences, which is essential in ML systems. - from https://ieeexplore-ieee-org.galanga.hvl.no/document/9609199 - refer challenges table 
%\keila{Discuss the fact that this is a long-term process the goal is to have research-based innovation not so much focus on time to market. Hence, the bi-annual meeting with all the stakeholders has been a feedback and validation step for the work conducted.}
% Software and data system-dependent quality attribute relation 
% "light trade-off analysis"

%strong inclination to reliability and availability
%if we consider the context of the architecture, then integrability must also be taken into account, although some factors are shared with interoperability in the ISO model

%“data quality by design”

%the degree which data quality affects software quality and vice-versa

%System that receives data from heterogeneous sources depending on the number of data producing sysmtes they integrate.
% \subsection{Data Flows}
% \label{sec:flows}
\section{Discussion} %Lessons Learned
\label{sec:discussion}
% Governance implications - conflicts in PROFES'22 paper
%In this section we describe the different flows of data, complementing the description of the components done in Section~\ref{sec:decisions} in the overall software architecture depicted in Figure~\ref{fig:arch}. 



At the Underwater Wireless Sensor Network (UWSN) level, the components are managed by the organization that developed and deployed them as a service. These systems are responsible for delivering data further up until the decision-making side at the \textsf{Data Consumer Application}. 
Because of the custom hardware setup of the data producers’ systems, the data can flow among the processing and transmitting components, traversing different traces according to the routing protocols inside the UWSN. From the data producer actor viewpoint, the components at this level must optimize the data to be sent up, prioritizing what is more relevant for the operations in case there are conflicts in the bandwidth usage. At the same time, there is a need to balance the battery consumption, the environmental impact of the data delivery in (near) real-time, and the network security measures (\textbf{AD1}). 

Regarding the cross-cutting concerns at UWSN level, on the one hand, the data producer systems are able to remotely monitor and configure the different nodes. 
%To implement this behavior, local agents are also needed to collect information on the nodes state and to interpret the commands coming from control stations in the opposite direction of the marine data flow delivery. 
On the other hand, concerning the security, there are no domain-specific solutions to address the challenge of securing underwater wireless communications in the case of obstruction of the communication channels (denial-of-service), or a compromised node (spoofing) since the wireless communication channels underwater is open. Solutions used on other wireless communication and IP networks can be deployed but the constraints in the systems' resources capacity must be taken into account. 
%Furthermore, the likelihood of attacks should also be considered in the risk assessment when specifying the requirements according to the degree of ``sensitivity'' of data being collected and transmitted at the UWSN level.
%\paragraph{Cloud} 
% ingested data sources processing -> deliver everything in the same format by the end of the processing pipeline - common understanding from heterogenous data.

At the cloud level, the  \textsf{\small Ingested Data Processing} sub-components are loosely coupled for the elasticity of the computation due to the variable volume of data pushed or pulled into the pipeline. Additionally, data might need different processing services according to its quality. 
The first step into the processing of heterogeneous data streams ingested is to convert them to a complying syntax and semantics, assuring that all the processing components work upon the same specification and understanding of data (\textbf{AD7}). This step is also responsible for validating the ingested data, contributing to the completeness and compliance quality attributes of data. If the storage of data in its raw format is desired for future reprocessing, this can be achieved by the proposed architecture. % proposed in Figure~\ref{fig:arch}.
After the transformation process, data is again ingested into the \textsf{\small Core
Broker} component for distribution to the different  \textsf{\small Stream Processing} services. Additional information might be need by these processing services not only at the UWSN level but also from external data. Another responsibility held by the  \textsf{\small Stream Processing} component is the categorization of data, aiding the sharing access control rules implementation.
%\thanh{Seems irrelevant, suggest to remove.}\keila{This is related with AD10}\thanh{I guess you want to keep it?}
The data model will be have a great impact into the selection of solutions for the database management system (\textsf{\small Data Space} component in Figure~\ref{fig:arch}). It is important to have a flexible database model to minimize the overload when updating the components with the evolution of the data and metadata fields requirements.

Regarding the cross-organizational data flow, to enable the flexibility on the delivery of data needed at the cloud side, there are three traces for data ingestion in the data management layer. In the proposed architecture, this can be achieved via the pusher, fetcher or the edge components.
The first component is responsible to integrate data sources at the cloud level interacting with data producers' systems over IP networks. In this case of data ingestion, the responsibility lays on the data producers side to push data into the data management layer.
Second, the  \textsf{\small Data Fetcher} component can pull data from ephemeral data acquisition systems (manual/ship sea surveys), other databases or streams into the processing pipeline.
Thirdly, the \textsf{\small Edge Integration Management} component differs from the others in its physical location at the UWSN level. In this case, the data sources integration is performed closer to the data acquisition, with more access to information in this layer, transferring the costs of OTA transmissions done via the  \textsf{\small Network Carrier Gateway} component. For this component to be implemented, the data producers' systems have to be exposed for integration locally.
%with an external system in the data actor viewpoint of the organization operating the sensing platforms.
The existence of neither one of these three components is exclusive, this is a reflection of the distribution of processing and communication responsibilities in the first architectural decision (see Table~\ref{tab:decisiosn}), as was demonstrated in the architecture implementation in Figure~\ref{fig:prototype}.% (see Section~\ref{sec:prototype_arch}).

%among the data management layer, the UWSN and the \textsf{Data Consumer Application}
Finally, on the cross-organizational data flow, there is a need to make heterogeneous components' authentication methods uniform to enforce ingestion access policies and sharing rules. There is also a need to regulate the access to data via push and pull methods (from the  \textsf{\small Stream Processing} or the  \textsf{\small Data Space} respectively), in similarity to the ingestion of that into this data management layer. These concerns are transversal to the architecture and must be implemented in the organizational boundaries along the data flow.
%
%Finally, on the cross-organizational data flow between the data management layer and the \textsf{Data Consumer Application}, there is a need to make heterogeneous components authentication methods uniform to ensure the enforcement of the sharing rules and policies to operations and decision-making systems, regulatory data delivery, or data reusability in open-data platforms. This component is also needed to regulate the access to data with push and pull methods (from the \textsf{Stream Processing} or the \textsf{Data Space} respectively), in similarity to the ingestion of that into this data management layer. Those rules and policies are implemented via the \textsf{Access Control} component.

==> sections/method_Thanh.tex <==
\section{Research methodology} %\thanh{Done. Ready for review.}
\label{sec:method}
Our study is motivated by a real-world need for a software architecture accommodating wireless smart ocean observation systems (hereafter, referred to as \texttt{System}). %, as described in Nguyen et al.~\cite{ref14}. %That paper discussed challenges of building \texttt{System} through the lens of software engineering and is the starting point of our study. 
%\rogardt{Is not the design circle called evaluation circle?}
We follow the Design Science approach~\cite{hevner2010design} to conceive and design %the software architecture for \texttt{System}. The novelty of this study consists of %the artifacts, including 
the architectural decisions (Section~\ref{sec:decisions}) and the software architecture for \texttt{System} (Section~\ref{sec:prototype_arch}), which address our identified real-world problem. 
%They have been % artifacts were 
%derived via a %from our 
%research process based on relevance, rigor, and design cycles (Section~\ref{sec:method_process}). 

%Subsequently, we elaborate on how we have followed Design Science in the study.
% methodology, specifically following the structure outlined by Hevner (ref) with the relevance, rigor, and design circles. The uniqueness of this paper lies in both the process and the artefacts derived from it, enabling us to acquire rationale, architectural decisions, and the architecture for marine ocean applications.
%\ins{We will start by examining the context, which plays a pivotal role in design science. Following that, we will elaborate on how we adhere to the various phases or stages within the design science methodology.}
%\del{Subsequently, we introduce the context of our research and then explain the research process that we followed conceive the Smart Ocean architecture.}
% depicts how we follow the Design Science in Information Systems Research approach~\cite{hevner2010design} to conceive the Smart Ocean architecture.

\subsection{Context}
\label{sec:context}

%Our study closely links to industry. To ensure that its outcomes sufficiently address industry needs, it is important to consider research context~\cite{petersen2009context}. Developments of SE artifacts need to consider real-world requirements and constraints through collaborations with practitioners to maximize their impact~\cite{briand2012embracing,briand2017case}. There is no universal solution for industrial software engineering (SE) research~\cite{dybaa2012works}. 

The research context plays a crucial role in Design Science~\cite{petersen2009context}. %and Software Engineering research
%~\cite{petersen2009context}. 
Our study involves %is comprised of 
16 marine organizations that collaborate %have a common interest 
to build \texttt{System}, as detailed in Table~\ref{tab:partners} (gray rows indicate software-related stakeholders). \texttt{System} accommodates representative use cases within ocean industries covering aquaculture, environmental monitoring, and energy. The stakeholders play different data-related  roles in building \texttt{System}: 

%as detailed below:  %In Table~\ref{tab:partners} we present the organizations with whom the collaboration is being done. All the stakeholders involved in the main three activities conducted throughout the research process belong to these organizations. 
\begin{table}[!t]
  %\begin{threeparttable}
  \caption{Organizations involved in building \texttt{System}}
  \label{tab:partners}
  {\footnotesize
  \begin{tabular}{|p{.20cm}|p{.8cm}|p{5.3cm}|p{0.9cm}|}
    %\toprule
    
    %\midrule
    \hline
    \textbf{ID} & \textbf{Size}     & \textbf{Profile }    & \textbf{Role}   \\
       & \textbf{(emp.)} &          &       \\
\hline
    %1       & $<$250    & Physics and technology research group expert in acoustics. & \\
    %\hline % UiB
    1       & $<$250    & Producer of oceanographic sensors and supplier of sensory services & P, S, C\\
    \hline % Metas
    \cellcolor{gray!40} 2       & \cellcolor{gray!40} $>$250    & \cellcolor{gray!40} Research institute on technology development for sensors and decision support & \cellcolor{gray!40} C\\
    \hline % NORCE
    \cellcolor{gray!40} 3       & \cellcolor{gray!40} $>$250  & \cellcolor{gray!40} Underwater communication and marine robotics manufacturer  & \cellcolor{gray!40} P, S \\ % Kongsberg
    \hline
    4      & $>$250  & Defence-related research and development institute  &  P, S \\ % FFI
    \hline
    5     & --  & Marine industry cluster to foster technology synergies in the sector &  I \\
    \hline % GCE OCEAN Tech
    6  & $>$250 & Oil exploration and petroleum resources development company &  C  \\ % AkerBP
    \hline
    \cellcolor{gray!40} 7  & \cellcolor{gray!40} $<$250 & \cellcolor{gray!40} Oceanographic sensors manufacturer and sensor services provider &  \cellcolor{gray!40} P, S  \\ % AADI
    \hline
    \cellcolor{gray!40} 8     & \cellcolor{gray!40} $<$250  & \cellcolor{gray!40} Manufacturer of underwater communication systems and monitoring services provider & \cellcolor{gray!40} P, S  \\
    \hline % Wsense
    \cellcolor{gray!40} 9      & \cellcolor{gray!40} $>$250  & \cellcolor{gray!40} IT and digital solutions consultancy &  \cellcolor{gray!40} S, C  \\
    \hline % Bouvet
    10      & --  & Innovation industry cluster to foster national and international R\&D cooperation &  I \\
    \hline % GCE NODE
    11     & $<$250    & Research institute focus in marine, cryospheric and atmospheric studies &  P, S, C \\
    %\hline % NERSC
    \hline
    12      & $>$250  & Subsea systems development, operation, and consultancy &  P, S  \\
    \hline % Reach Subsea
    \cellcolor{gray!40} 13     & \cellcolor{gray!40} $>$250  & \cellcolor{gray!40} Marine research institute    &  \cellcolor{gray!40} P, S, C \\
    \hline % IMR
    14      & $<$250  & Offshore telecommunications carrier &  S  \\
    \hline % Tampnet
    15     & --  & Cluster of research institutes, governmental bodies, companies related to seafood industry  &  I, C  \\% Seafood Innovation
    \hline
    16      & $<$250  & Subsea inspection systems development and operation &  P, S  \\
    \hline % TSC Subsea
    %\bottomrule 
\end{tabular}
}
%    \begin{tablenotes}
%      \item \footnotesize
     %\hspace{.1cm}
%	 - P: Data Producer / S: Data Service Provider / C: Data Consumer / I: Industry cluster for innovation and knowledge transfer
  %Bridging organizations for knowledge transfer between research and industry settings. 
%    \item \footnotesize - Gray rows indicate software-related stakeholders.%\keila{Considering the GCE Node email response, we can maybe adapt the description to their answer and the SFI partners description: Sector representatives functions as knowledge transfer organizations, bridging the gap between developments within a research and an industrial setting.}\thanh{Call it ``Bridging organizations for research and industry settings''?}
%    \end{tablenotes}
%\end{threeparttable}
\vspace{-0.5cm}
\end{table}


%As for the organizations' roles process for building the overall system, we have divided them into:
\begin{itemize}
    \item \textbf{Data Producers} (Role \textbf{P}): organizations responsible for developing and integrating underwater sensors into Underwater Wireless Sensor Networks (UWSNs).% \thanh{Don't know if UWSN will be mentioned somewhere later. If not, just remove to not confuse readers and complicate the work}.% to . They are expected to establish a UWSN to transmit data from the ocean to the cloud where data management platforms are situated.
    %\keila{It is currently used in the architecture figure and in many places when describing components and challenges related to the network layer.}
    
    %component of the overall Internet-of-Underwater Things (IoUT). These types of organizations are also responsible for delivering data into the cloud side, creating a bridge from the underneath wireless sensor network layer (edge and fog devices) of typical IoT system architecture.
    \item \textbf{Data Service Providers} (Role \textbf{S)}: organizations providing services for transmitting, processing, or sharing data in underwater and onshore environments. %organizations providing wireless communication networks in both underwater and onshore environments. %services throughout the data delivery chain, whether it is telecommunication-related, software-related, or both. These organization does not necessarily need to produce data but in the case of the data producers, they can have services to deliver the data to the cloud side. These services comprise any software system in place that facilitates the transmission, processing, and access to data collected by data producers.
    \item \textbf{Data Consumers} (Role \textbf{C}): organizations consuming data produced by \texttt{System} for data analytics purposes. They provide crucial requirements for building an architecture that can be parameterized for specific use cases.
    \item \textbf{Industry Clusters} (Role \textbf{I}): clusters of organizations that take responsibility for one or more of the three roles described above, but do not directly involve themselves in building \texttt{System}. The clusters are responsible for knowledge and technology transfer between research and the industrial settings to support innovation.
\end{itemize}

\subsection{Research process}\label{sec:method_process}
Figure~\ref{fig:research_process} depicts the relevance, rigor, and design cycles following the Design Science research approach~\cite{hevner2010design}.

\begin{figure}[h]
  \centering
  %\includegraphics[width=\linewidth]{figures/rq2_reviewed.pdf}
  % [trim={left bottom right top},clip]
  \includegraphics[trim={6.2cm 2.5cm 3cm 2cm},clip,width=\linewidth]{figures/method/research_method_sys.pdf}
  \vspace{-.4cm}
  \caption{Research process with: a) depicting the relevance cycle; and b) illustrating the rigour cycle and solution design process}%keila{Maybe we can change "SW Prototyping" with "Prototype" because it is an output and not an activity. Also, the rationale can be incorporated into the architectural decision by definition and maybe we can replace it by ``QA analysis''.}\thanh{How about ``SW prototype''? as it is not clear for me the output of prototype. About the 2nd point, my idea is to map our contributions to specific sections in the paper. I cannot see QA analysis but only architecture decisions. As you merged architectural rationales into architectural decisions (if I remember correctly), it is fine for me to call architectural decisions. BTW, I do not see you mention much about existing software technologies mentioned in the architecture. Do you plan to so? Otherwise, we have to think a bit about the input.}
  \label{fig:research_process}
  %\vspace{-.5cm}
\end{figure}

\textbf{Relevance cycle:} Figure~\ref{fig:research_process}a illustrates how we, the architect team, ensure that the produced artifacts are relevant to the needs of the stakeholders listed in Table~\ref{tab:partners}. %regarding the software architecture accommodating \texttt{System}. 
The relevance cycle of this study started in January 2022. Each team member worked individually and the whole team gathered for 2 hours every week, for status updates and to discuss issues encountered while producing the artifacts. We also organized 2-hour monthly workshops with the software-related stakeholders. These workshops aimed to elicit the software requirements, determine the architecture to be developed, identify necessary architectural decisions, and validate our ongoing efforts. The artifacts were presented in 2-day bi-annual workshops bringing together all stakeholders of the project together. The primary aim of the bi-annual workshops was to ensure the alignment of all the software architecture's components of \texttt{System}, including underwater data acquisition, network communication, and software technologies. 
%that the software architecture of \texttt{System} aligns with all of its components \lars{what does "aligns" mean here?}, including underwater data acquisition, network communication, and software technologies. 

%\textbf{Rigor cycle:}

\textbf{Rigor and Design cycles:} Figure~\ref{fig:research_process}b shows the cycles of rigor and design. %Regarding the rigor cycle, 
We took into account the challenges of building smart ocean observation systems presented in the literature (Section~\ref{sec:challenges}), and existing software technologies (Section~\ref{sec:decisions} and~\ref{sec:prototype_arch}). Those findings resulted in decisions and a software architecture for \texttt{System} (Sections~\ref{sec:decisions} and~\ref{sec:prototype_arch}). A prototype implementation of the software architecture was made to validate the decisions and adjust them accordingly. Details of the software components can be found in our replication package~\cite{replication_package}.

%In Figure B, you can observe the evaluation process conducted within the architecture team. Architecture decisions are founded upon the identified challenges, leading to the creation of an architecture, followed by the development of a prototype to validate this architecture. Hence, the novelty of this paper lies in the validation of architectural decisions. This validation occurs internally through our iterative process and is further substantiated by discussions during our monthly and biannual meetings. \rogardt{Should we say something about this being very much an agile process}

%\textbf{Rigor cycle:}

%\subsubsection{Relevance Cycle}
%\chg{Figure A shows that the architecture team involved in this research conducts weekly meetings, each lasting 2 hours.} {A single architecture team generated the artefacts presented in this paper. Figure A illustrates how the architecture team acquired information to and from the context described in the previous subsection.} \del{Additionally,} \chg{w}{W}e organise monthly software-related workshops where we engage with stakeholders from  \rogardt{various areas seems a bit to informal, we should be a bit more concrete} various areas. These workshops aim to comprehend the software requirements, determine the architecture to develop, identify necessary architectural decisions, and validate our ongoing efforts. Moreover, biannually, we convene the entire consortium. These biannual meetings aim to gain a comprehensive understanding of our software solution within a larger contextual framework.
 
%\subsection{Rigor Cycle}
%\rogardt{Following Hevner's approach (ref), acquiring knowledge from the knowledge base and bringing it back is essential. This process is facilitated through the rigour circle.}
%All the architectural challenges discussed in this paper are derived from the references cited ... . These challenges are presented in Figure X. They are primarily deliberated upon during our weekly meetings, where architectural decisions are discussed to address these challenges. Furthermore, these challenges are validated within our monthly workshops. \ins{We also have a number of tools coming from the knowlege base ...}. \ins{What we bring back is ...} . \ins{Next subsection will ...}
 
%\subsection{Design Cycle} 
%In Figure B, you can observe the evaluation process conducted within the architecture team. Architecture decisions are founded upon the identified challenges, leading to the creation of an architecture, followed by the development of a prototype to validate this architecture. Hence, the novelty of this paper lies in the validation of architectural decisions. This validation occurs internally through our iterative process and is further substantiated by discussions during our monthly and biannual meetings. \rogardt{Should we say something about this being very much an agile process}

\iffalse
Firstly, during spring and autumn every year since 2022, all stakeholders are brought together in a 2-days seminar to discuss the latest advances and on the prototype which includes discussion on the hardware, software and telecommunication parts of the overall system. During these two days, there is also dedicated space to discuss each one of the parts of the system in depth.

Secondly, the monthly workshops conducted with the \textit{software-related stakeholders} fostered more technical discussions with representatives responsible for the systems involved in 
\rogardt{What is the data value chain, did we define that, or do you mean the design circle in the previous paragraph}
the data value chain. These representatives come from the organizations listed in Table~\ref{tab:partners} whose systems and/or data are integrated into a prototype wireless autonomous stationary marine observing system. In terms of duration, these workshops took around 2 to 2,5 hours. 

Lastly, in the internal team (authors) involved in the software architecture definition, and because the process is research-based, there is also input from literature besides the feedback from the different discussions with the stakeholders described above. In these meetings, the concerns captured from all inputs are translated into architectural decisions that are then implemented in new constituents, or integrated with the existing ones, tuning the decisions with the feedback from the \textit{prototyping} process.
When the prototype is tested and validated internally, then the \textit{validation} process starts up the stakeholders' chain in the two different workshops with the stakeholders and the \textit{feedback} received triggers a new cycle in the overall methodology process.
In summary, the following major activities were part of the methodology: 
\begin{itemize}
    \item Monthly workshops from the past 3 years from November 2020 to November 2023. % 19
    \item 2-day biannual seminars from Spring 2022 to Autumn 2023. %4
    \item Weekly meetings from January 2022 to November 2023. %many
\end{itemize}
%\keila{Add duration of meetings: 2hours}

The methodology described gives a high-level view of the process in enough detail to understand the research and development chain to the background and results presented in the following sections. Furthermore, activities such as threat analysis with different stakeholders in their integrated systems are also being taken and have aided in understating the boundaries between the different tiers and the data flow between them.
\fi

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

%\cite{abughazala2022dat} identifies i
Important aspects of data architecture for Internet-of-Things 
(IoT) applications are~\cite{abughazala2022dat}: data quality, data security, organizational efficiency, business intelligence and analytics, and scalability and flexibility. IoT is the foundation of IoUT in which \texttt{System} is situated~\cite{pena2005itu}. We took into account those aspects while designing our architecture.

Some software architectures have been proposed to accommodate heterogeneous aspects~\cite{seifermann2019data,rademacher2019aspect,CORRALPLAZA2020103426}. However, none of them considers a broad number of software and data quality concerns as we have identified, and neither a data actor viewpoint. ~\cite{seifermann2019data} deals with the confidentiality of multiple data streams. A metamodel built on top of the Architectural Description Language (ADL) Palladio Component Model (PCM)~\cite{reussner2016modeling} is proposed to detect access right mismatches regarding data consumption roles of an information system. This solution covers only two challenges (CH13 and CH15 in Table~\ref{tab:challenges}). In IoT environments, ~\cite{CORRALPLAZA2020103426} proposes an architecture focusing on the heterogeneous data processing layer based on nine requirements from 2 survey studies, abstracting the data sources and consumers.
~\cite{rademacher2019aspect} addresses the challenges of accommodating various different technologies used in information systems. There are different software technologies utilized in our software architecture (see Section~\ref{sec:decisions}). We rely on Service-oriented Architecture (SOA)~\cite{siqueira2021service, hastbacka2019dynamic} to decouple the components and let stakeholders take responsibility of maintaining their components independently. We leverage MQTT as a plug and play mechanism~\cite{hastbacka2019dynamic} to facilitate migrations of various data sources to the system and address the challenge of having multiple communication protocols, data formats, and data streams in \texttt{System}.%, being inline with.

%The more sensors and data sources integrated into data streams, the more data format and semantics, and communication protocols that an integration system has to deal with. Being inline with~\cite{hastbacka2019dynamic}, we leveraged MQTT as a plug and play mechanism to facilitate migrations of various data sources to the system and address the challenge of having multiple communication protocols in \texttt{System}. %To deal with heterogeneous data formats, we developed a data transformation module to ensure that all data coming out from the system will eventually be represented in a unified format. 
%As \texttt{System} have many independent and self-serviced components, we rely on Service-oriented Architecture (SOA)~\cite{siqueira2021service, hastbacka2019dynamic} to decouple the components and let stakeholders take responsibility of maintaining their components independently. 
%We leveraged the REpresentational State Transfer (REST) technology to enable data communication between different data streams from various organizations. 
%\thanh{The paper also discuss SOA but not sure if it worth mentioning here for now. There are to me enough recipes for related work on that paper.}

%Our work takes into account factors affecting the quality of systems (detailed in~\cite{ref13}) and data (see~\cite{ref15}) for a data platform accommodating multiple marine data sources. To ensure that we have captured all challenges for \texttt{System}, we survey the literature

% \thanh{\chg{Concerning the analysis of concerns from the domain that influence the overall system quality attributes, while in~\cite{ref13} there is an analysis of the software-related ones, in ~\cite{ref15} there is an analysis of data quality requirements concerning 9 different marine use cases. In our study, we analyse domain-specific concerns inferred from challenges analysing the software and data quality related attributes with a wider range of concerns as a result of the gathering of challenges from literature. Moreover, in the IoUT domain, another study has proposed 3-layered architecture from a process iterating between design, implementation, and validation~\cite{RAZZAQ2023100893}. In the referred work concerns were elicited from multi-vocal literature having implementation of the proposed architecture validation in terms of three runtime performance efficiency metrics (throughput, CPU utilization and query response time) following the same software quality model. Our work differentiates from this one by considering in the resulting architecture heterogeneous data streams adding an extra layer of complexity in the processing and usage of data. Furthermore, we have addressed not only software quality and also data quality concerns into the design of the system.}
% {\cite{RAZZAQ2023100893} proposes an architecture for an IoUT system and validates the runtime performance efficiency with three metrics: throughput, CPU utilization, and query response time. We design our architecture to accommodate heterogeneous data streams and check if the associated challenges are sufficiently addressed or not. To do so, we survey the literature with the starting point from~\cite{ref14}.\thanh{Keila, you wrote some texts describing how you surveyed the literature for challenges. It would be a good idea to put it here.} At the end, we take into account factors affecting the quality of not only software (like~\cite{ref13}) but also data (see~\cite{ref15}) while designing the architecture.}}

% \chg{\cite{RAZZAQ2023100893} proposes an architecture for an IoUT system and validates the runtime performance efficiency with three metrics: throughput, CPU utilization, and query response time.}
% {A recent proposal of an architecture for an IoUT system validates the runtime performance efficiency with three metrics: throughput, CPU utilization, and query response time \cite{RAZZAQ2023100893}.}
% \del{We design our architecture to accommodate heterogeneous data streams and check whether the associated challenges are sufficiently addressed.} 
% While their method is based on four multi-vocal references, our work has a concrete context that was considered alongside challenges gathered in literature, which resulted in nineteen studies. 
% \ins{Consequently, our validation focuses on the specific challenges rather than metrics, allowing us to} 
% \del{Overall, we} take into account factors affecting the quality of not only software (like~\cite{ref13}) but also data (see~\cite{ref15}) while designing the architecture.

%A recent proposal of an architecture for an IoUT system validates the architecture's runtime performance efficiency with three metrics: throughput, CPU utilization, and query response time \cite{RAZZAQ2023100893}.While their method is based on four multi-vocal references, 
More recently, an architecture for an IoUT system has been proposed based on four multi-vocal references and validated with three quantitative performance efficiency metrics~\cite{RAZZAQ2023100893}.
Our work has a concrete context that was considered alongside challenges gathered in literature, which resulted in nineteen studies.
Consequently, our validation focuses on the specific challenges rather than metrics, allowing us to
take into account factors affecting the quality of not only software (like~\cite{ref13}) but also data (see~\cite{ref15}) while designing the architecture.


%~\cite{abughazala2022dat} identifies important aspects of a data architecture, namely: data quality, data security, organizational efficiency, business intelligence and analytics, and scalability and flexibility. In our case, 

%https://www.sciencedirect.com/science/article/pii/S0169023X2300012 - data quality by design and context dependent difficult task
%
% Similarities and Differences with Smart City
%\keila{Papers on architecture with similar constraints - low bandwidth and battery}
%
%https://ieeexplore.ieee.org/abstract/document/8956662?casa_token=bFVscvIWPUUAAAAA:AhRjYajpttkaw6pdMC4ASmbDdmUoXkOVV6sL0fFdBuyS1dLKkU1sVlej4Q4dA3f_WnqVOCP9
%
%https://dl.acm.org/doi/epdf/10.1145/3478680
%
%https://ieeexplore.ieee.org/abstract/document/9095740
%
%DFD - https://ieeexplore.ieee.org/abstract/document/8703923?casa_token=RQeAMutDeHsAAAAA:j6gZ3HXEtgat9ryNRdK6srcs89HJadbcp80_VwnBA7Z8qj6Yc0ZQQ9u0XQGgcYQn9MjDrIFoERY
%
%https://link.springer.com/chapter/10.1007/978-3-030-67270-6_3
%
%https://ieeexplore.ieee.org/abstract/document/10092619?casa_token=4dM_zIjMi98AAAAA:vaC1urZ-OoXncNVie9SNGkKTV6nWArTLEvK0kq6x3fKp7XSzft0pa-0BuB7YQzvPTb3jVnif3-A
%
%https://www.sciencedirect.com/science/article/pii/S0167739X2300345X?casa_token=wVbyjj3LTCoAAAAA:Ofu6oYv39XAGe7NwOemVZXSF3AX157425MCqZh6JGP09WnlQwnnvjZSSFiNxHDo0QPD8pDDXgw
%
%https://www.diva-portal.org/smash/record.jsf?pid=diva2%3A1790842&dswid=8354



==> sections/validity.tex <==
\subsection{Threats to validity}\label{sec:validity}
% Argue for ad hoc selection of papers for challenges gathering -> domain knowledge gain in the past years
% IoTJ paper references in table 5 and latest papers refering them because since they were surveys there is no point on going on its references
%Many of the Papers are surveys or challenges gathering in venues used by researchers and practicioners in the domain 
% Mention the lack of end user applications on top of the data platform (in the current implementation)
%Below we discuss potential threats to the validity of the approach employed in this study.
%expertise is perceived as KB in our research methodology paradigm in Hevner
\subsubsection{Construct Validity}
 Since the gathered challenges from the literature were a pivotal point in our research methodology, we do not claim to have identified all the existing challenges for data-driven systems that process marine in-situ data in realtime. We focus on the ones that our architectural decisions address in the intersection of our design cycle, the rigor cycle outcomes, and the relevance cycle inputs and validation. While the authors gained domain knowledge, gathering papers in the literature diminished until the understanding of the challenge reached a saturation point. Furthermore, to analyse the challenges, we use standardized quality models, which were extended by inserting minimal changes (two additional quality attributes) supported by the literature.

\subsubsection{Internal Validity}
To reduce the threat of misinterpretation of the identified challenges, we used views from different reference papers from literature collected over the research period. To validate the rationale behind the challenges, they were discussed several times with the stakeholders in the activities held in the relevance cycle (see Figure~\ref{fig:research_process}a).
We proposed an architecture that reflects the decisions whose rationale incorporates existing challenges from different studies, technological solutions, and stakeholders' domain expertise. 
Furthermore, we do not limit the validation of the resulting architecture to the stakeholders' interaction chain; we also integrate feedback from the prototype technical implementation process. The integration and prototyping processes only started when sufficient knowledge of the domain was acquired to ensure that as many factors as possible were taken into consideration in the solution-seeking stage.

\subsubsection{External Validity}
The research process focused on requirements for a set of heterogeneous data-driven use cases within the marine domain. Our resulting flexible and parameterized architecture is a reflection of this.
Consequently, in contexts that share similar challenges as those described throughout Section~\ref{sec:challenges}, the related architectural decisions can be suitable for similar systems. 
%The generalization of the results could potentially include energy-constraint IoT-enabled systems in other application domains that operate in remote areas of public interest in terms of their impact on livelihood, defense, or resource provision.  %High maintanance and deployment costs
%air and space
Lastly, the architectural decisions entail some limitations, and their usage in other contexts has to be analyzed carefully to ensure the quality of the resulting architecture.

\subsubsection{Reliability}
To improve the reliability of the study, we provide the documents from which Tables~\ref{tab:challenges} and~\ref{tab:decisiosn} were extracted. As for the resulting architecture, we also provide the initial draft upon which new knowledge has been integrated between the many iterations over our relevance, design and rigor cycles (Section~\ref{sec:method}). Because of intellectual property rights (IPR) constraints and the cross-organizational context, the source code of the end-to-end prototype implementation cannot be provided. Runtime excerpts of the system's operation is provided. All this data is available in the replication package of the study in~\cite{replication_package}\footnote{This package data will be published officially in Zenodo once the anonymization of authors is no longer required}.
%and more information of architecture in context can be provided when the authors identity can be disclosed.
